Type Ia Supernovae are Good Standard Candles in the Near Infrared: Evidence from PAIRITEL

We have obtained 1087 NIR (JHKs) measurements of 21 SNe Ia using PAIRITEL, nearly doubling the number of well-sampled NIR SN Ia light curves. These data strengthen the evidence that SNe Ia are excellent standard candles in the NIR, even without correction for optical light-curve shape. We construct fiducial NIR templates for normal SNe Ia from our sample, excluding only the three known peculiar SNe Ia: SN 2005bl, SN 2005hk, and SN 2005ke. The H-band absolute magnitudes in this sample of 18 SNe Ia have an intrinsic rms of only 0.15 mag with no correction for light-curve shape. We found a relationship between the H-band extinction and optical color excess of AH=0.2E(B-V). This variation is as small as the scatter in distance modulus measurements currently used for cosmology based on optical light curves after corrections for light-curve shape. Combining the homogeneous PAIRITEL measurements with 23 SNe Ia from the literature, these 41 SNe Ia have standard H-band magnitudes with an rms scatter of 0.16 mag. The good match of our sample with the literature sample suggests there are few systematic problems with the photometry. We present a nearby NIR Hubble diagram that shows no correlation of the residuals from the Hubble line with light-curve properties. Future samples that account for optical and NIR light-curve shapes, absorption, spectroscopic variation, or host-galaxy properties may reveal effective ways to improve the use of SNe Ia as distance indicators. Since systematic errors due to dust absorption in optical bands remain the leading difficulty in the cosmological use of supernovae, the good behavior of SN Ia NIR light curves and their relative insensitivity to reddening make these objects attractive candidates for future cosmological work.

==> full.tab5.tex <==
\begin{deluxetable}{lllrr}
\tablewidth{0pc}
\tablecaption{Light Curve Table Stub}
\tablehead{
\colhead{SN} & \colhead{MJD} & \colhead{Passband} & \colhead{Flux$_{25}$\tablenotemark{a}} & \colhead{Flux err$_{25}$} \\
}
\startdata
sn2005ao   &    53846.373 &        H &        -3.89 &         4.08 \\
sn2005ao   &    53845.428 &        H &        41.85 &        90.56 \\
sn2005ao   &    53901.216 &        H &        53.68 &        90.52 \\
sn2005ao   &    53844.480 &        H &       -63.41 &         3.49 \\
sn2005ao   &    53841.330 &        H &       -92.06 &        90.60 \\
sn2005ao   &    53842.355 &        H &       176.58 &        90.57 \\
sn2005ao   &    53464.387 &        H &       339.24 &       128.04 \\
sn2005ao   &    53466.388 &        H &       345.10 &        90.64 \\
sn2005ao   &    53481.485 &        H &       373.72 &       128.05 \\
sn2005ao   &    53456.430 &        H &       437.98 &         3.64 \\
sn2005ao   &    53467.385 &        H &       561.79 &         3.76 \\
sn2005ao   &    53440.416 &        H &       600.25 &         3.57 \\
sn2005ao   &    53469.409 &        H &       737.78 &       128.04 \\
sn2005ao   &    53470.368 &        H &       871.84 &         3.31 \\
sn2005ao   &    53887.264 &        H &      -180.52 &        90.65 \\
sn2005ao   &    53901.216 &        J &        49.12 &        32.00 \\
sn2005ao   &    53846.373 &        J &       -73.68 &        39.19 \\
sn2005ao   &    53466.388 &        J &       241.59 &        32.00 \\
sn2005ao   &    53456.430 &        J &       291.78 &        39.19 \\
sn2005ao   &    53464.387 &        J &       316.27 &        32.00 \\
sn2005ao   &    53467.385 &        J &       388.07 &        22.63 \\
sn2005ao   &    53473.351 &        J &       396.39 &        45.25 \\
sn2005ao   &    53440.416 &        J &       692.00 &        50.60 \\
sn2005ao   &    53901.216 &       Ks &         0.16 &         3.62 \\
sn2005ao   &    53842.355 &       Ks &        55.22 &       256.15 \\
sn2005ao   &    53481.485 &       Ks &       -38.82 &       181.44 \\
sn2005ao   &    53845.428 &       Ks &       -67.32 &       256.15 \\
sn2005ao   &    53887.264 &       Ks &       212.52 &       256.20 \\
sn2005ao   &    53467.385 &       Ks &       240.78 &       181.39 \\
sn2005ao   &    53464.387 &       Ks &       264.83 &       181.30 \\
sn2005ao   &    53846.373 &       Ks &       381.68 &       256.32 \\
sn2005ao   &    53440.416 &       Ks &       559.45 &         7.57 \\
sn2005ao   &    53469.409 &       Ks &       767.09 &       181.24 \\
sn2005ao   &    53451.472 &       Ks &       792.62 &       256.33 \\
sn2005ao   &    53885.257 &       Ks &      -121.61 &       256.36 \\
sn2005ao   &    53841.330 &       Ks &      -310.58 &       256.42 \\
sn2005ao   &    53844.480 &       Ks &      -488.44 &       181.22 \\
sn2005ao   &    53470.368 &       Ks &      1089.15 &       181.31 \\
sn2005ao   &    53456.430 &       Ks &      1877.66 &       543.83 \\
sn2005bl   &    53480.162 &        H &       833.38 &        97.86 \\
sn2005bl   &    53481.223 &        H &      1010.35 &        79.48 \\
sn2005bl   &    53486.198 &        H &      1000.36 &       129.18 \\
sn2005bl   &    53487.177 &        H &      1165.13 &        99.65 \\
sn2005bl   &    53488.178 &        H &      1174.52 &        73.81 \\
sn2005bl   &    53490.162 &        H &       923.11 &       123.11 \\
sn2005bl   &    53493.168 &        H &       895.16 &        85.48 \\
sn2005bl   &    53494.137 &        H &       916.31 &        66.83 \\
sn2005bl   &    53497.164 &        H &       535.84 &        94.61 \\
sn2005bl   &    53498.147 &        H &       599.97 &        48.90 \\
sn2005bl   &    53502.142 &        H &       134.03 &        69.83 \\
sn2005bl   &    53503.142 &        H &       263.90 &        74.07 \\
sn2005bl   &    53506.127 &        H &       302.90 &        80.23 \\
sn2005bl   &    53515.236 &        H &        -6.77 &        41.30 \\
sn2005bl   &    53770.357 &        H &       -12.84 &        51.20 \\
sn2005bl   &    53480.162 &        K &       615.31 &       115.74 \\
sn2005bl   &    53486.198 &        K &       770.28 &       151.77 \\
sn2005bl   &    53490.162 &        K &      1028.98 &       133.81 \\
sn2005bl   &    53494.137 &        K &       297.04 &       143.17 \\
sn2005bl   &    53497.164 &        K &       677.49 &       136.03 \\
sn2005bl   &    53498.147 &        K &      -198.37 &       126.59 \\
sn2005bl   &    53502.142 &        K &      -114.96 &       106.65 \\
sn2005bl   &    53503.143 &        K &       125.38 &        44.70 \\
sn2005bl   &    53504.143 &        K &       -52.20 &       183.72 \\
sn2005bl   &    53515.236 &        K &      -255.60 &       177.38 \\
sn2005bl   &    53770.357 &        K &        -1.79 &        87.29 \\
sn2005bl   &    53480.162 &        J &       918.56 &        44.85 \\
sn2005bl   &    53481.223 &        J &       924.76 &        59.82 \\
sn2005bl   &    53486.198 &        J &      1011.57 &        49.15 \\
sn2005bl   &    53487.177 &        J &      1147.36 &        41.04 \\
sn2005bl   &    53488.178 &        J &       968.45 &        48.19 \\
sn2005bl   &    53489.168 &        J &      1086.24 &        57.74 \\
sn2005bl   &    53490.162 &        J &      1038.90 &        49.71 \\
sn2005bl   &    53493.167 &        J &       742.18 &        40.31 \\
sn2005bl   &    53494.137 &        J &       702.39 &        31.66 \\
sn2005bl   &    53497.164 &        J &       617.47 &        20.32 \\
sn2005bl   &    53498.147 &        J &       560.81 &        28.91 \\
sn2005bl   &    53502.142 &        J &       420.21 &        21.80 \\
sn2005bl   &    53503.142 &        J &       320.38 &        19.75 \\
sn2005bl   &    53506.127 &        J &       390.43 &        23.27 \\
sn2005bl   &    53515.236 &        J &       206.29 &        12.63 \\
sn2005bl   &    53770.357 &        J &        -8.89 &        26.57 \\
sn2005cf   &    53522.243 &        H &     13442.19 &       232.14 \\
sn2005cf   &    53523.245 &        H &     15784.69 &       443.76 \\
sn2005cf   &    53524.240 &        H &     18947.60 &       535.45 \\
sn2005cf   &    53539.209 &        H &     21307.14 &      1095.15 \\
sn2005cf   &    53536.209 &        H &     21672.28 &       676.18 \\
sn2005cf   &    53535.218 &        H &     21979.12 &       284.92 \\
sn2005cf   &    53563.146 &        H &     23014.59 &       447.31 \\
sn2005cf   &    53554.167 &        H &     23289.44 &       702.27 \\
sn2005cf   &    53556.165 &        H &     23683.80 &       381.16 \\
sn2005cf   &    53534.228 &        H &     24299.53 &       809.41 \\
sn2005cf   &    53560.157 &        H &     24336.04 &       410.60 \\
sn2005cf   &    53557.151 &        H &     24989.85 &      1855.41 \\
sn2005cf   &    53558.149 &        H &     25030.57 &      2048.00 \\
sn2005cf   &    53555.280 &        H &     25062.19 &      1374.49 \\
sn2005cf   &    53551.162 &        H &     25223.38 &      1476.28 \\
sn2005cf   &    53553.172 &        H &     25958.09 &      1494.92 \\
sn2005cf   &    53532.231 &        H &     25996.22 &       550.18 \\
sn2005cf   &    53551.162 &        J &      7291.90 &       170.17 \\
sn2005cf   &    53553.172 &        J &      7487.20 &       196.03 \\
sn2005cf   &    53554.167 &        J &      7540.93 &       161.44 \\
sn2005cf   &    53555.280 &        J &      7833.08 &       130.29 \\
sn2005cf   &    53556.165 &        J &      8083.60 &       174.19 \\
sn2005cf   &    53558.149 &        J &      8669.61 &       286.97 \\
sn2005cf   &    53557.151 &        J &      8778.41 &       186.25 \\
sn2005cf   &    53560.158 &        J &     10433.90 &       250.80 \\
sn2005cf   &    53563.146 &        J &     11965.69 &       264.47 \\
sn2005cf   &    53522.243 &        J &     13076.80 &       271.02 \\
sn2005cf   &    53523.245 &        J &     16147.68 &       226.00 \\
sn2005cf   &    53539.209 &        J &     18361.76 &       386.80 \\
sn2005cf   &    53524.240 &        J &     20151.07 &       515.71 \\
sn2005cf   &    53536.210 &        J &     23591.18 &       304.77 \\
sn2005cf   &    53534.228 &        J &     24538.52 &       991.01 \\
sn2005cf   &    53535.219 &        J &     25401.22 &       309.89 \\
sn2005cf   &    53532.231 &        J &     29384.91 &      1065.61 \\
sn2005cf   &    53522.243 &       Ks &     11924.28 &       234.05 \\
sn2005cf   &    53524.240 &       Ks &     18517.69 &       352.08 \\
sn2005cf   &    53551.162 &       Ks &     19928.65 &       356.26 \\
sn2005cf   &    53563.146 &       Ks &     20619.51 &       366.97 \\
sn2005cf   &    53553.172 &       Ks &     21600.84 &       346.43 \\
sn2005cf   &    53555.280 &       Ks &     21770.95 &       335.56 \\
sn2005cf   &    53556.165 &       Ks &     21998.63 &       419.92 \\
sn2005cf   &    53539.209 &       Ks &     22115.25 &       599.84 \\
sn2005cf   &    53560.158 &       Ks &     22600.32 &       427.17 \\
sn2005cf   &    53558.149 &       Ks &     23135.78 &       489.37 \\
sn2005cf   &    53557.151 &       Ks &     23283.90 &       232.85 \\
sn2005cf   &    53535.219 &       Ks &     23601.11 &       747.76 \\
sn2005cf   &    53536.210 &       Ks &     23869.46 &       420.42 \\
sn2005cf   &    53532.231 &       Ks &     25680.12 &       545.37 \\
sn2005cf   &    53534.228 &       Ks &     25937.24 &       361.39 \\
sn2005ch   &    53541.158 &        H &       913.67 &        80.01 \\
sn2005ch   &    53549.241 &        H &      1109.42 &        59.68 \\
sn2005ch   &    53550.145 &        H &      1042.27 &        52.85 \\
sn2005ch   &    53551.142 &        H &       967.44 &        56.49 \\
sn2005ch   &    53551.226 &        H &      1036.65 &        58.90 \\
sn2005ch   &    53556.200 &        H &      1034.38 &        77.93 \\
sn2005ch   &    53557.214 &        H &      1381.52 &        79.93 \\
sn2005ch   &    53558.213 &        H &      1419.68 &        82.42 \\
sn2005ch   &    53560.206 &        H &      1599.91 &        78.30 \\
sn2005ch   &    53563.217 &        H &      1594.76 &       101.85 \\
sn2005ch   &    53820.315 &        H &       -80.98 &        55.92 \\
sn2005ch   &    53823.441 &        H &      -960.42 &       346.69 \\
sn2005ch   &    53825.367 &        H &        97.57 &        36.63 \\
sn2005ch   &    53827.269 &        H &       -29.40 &        50.38 \\
sn2005ch   &    53829.312 &        H &      -214.71 &        88.77 \\
sn2005ch   &    53541.158 &        K &      1504.73 &       137.36 \\
sn2005ch   &    53550.145 &        K &      1232.92 &       100.12 \\
sn2005ch   &    53551.142 &        K &      1134.03 &       135.76 \\
sn2005ch   &    53551.226 &        K &       748.42 &       128.07 \\
sn2005ch   &    53556.200 &        K &      1639.15 &       131.46 \\
sn2005ch   &    53557.214 &        K &      1359.53 &       103.86 \\
sn2005ch   &    53558.213 &        K &      1369.31 &       119.30 \\
sn2005ch   &    53820.315 &        K &      -172.00 &        77.50 \\
sn2005ch   &    53823.441 &        K &     -2627.81 &      1564.52 \\
sn2005ch   &    53825.367 &        K &        65.19 &        98.03 \\
sn2005ch   &    53827.269 &        K &       125.89 &        74.10 \\
sn2005ch   &    53829.312 &        K &      3318.69 &       418.66 \\
sn2005ch   &    53541.158 &        J &      1019.41 &        53.58 \\
sn2005ch   &    53549.241 &        J &       325.64 &        26.10 \\
sn2005ch   &    53550.145 &        J &       241.77 &        19.89 \\
sn2005ch   &    53551.142 &        J &       311.18 &        25.19 \\
sn2005ch   &    53556.200 &        J &       396.04 &        25.28 \\
sn2005ch   &    53557.214 &        J &       475.01 &        22.22 \\
sn2005ch   &    53558.213 &        J &       388.82 &        24.13 \\
sn2005ch   &    53560.206 &        J &       474.53 &        26.42 \\
sn2005ch   &    53563.217 &        J &       594.72 &        35.27 \\
sn2005ch   &    53820.315 &        J &       -41.17 &        14.58 \\
sn2005ch   &    53823.441 &        J &       238.67 &        78.88 \\
sn2005ch   &    53825.367 &        J &        44.44 &        16.82 \\
sn2005ch   &    53827.269 &        J &        -3.55 &        10.02 \\
sn2005ch   &    53829.312 &        J &        88.87 &        35.15 \\
sn2005el   &    53708.293 &        H &       792.39 &        80.46 \\
sn2005el   &    53703.268 &        H &       928.73 &       111.87 \\
sn2005el   &    53703.268 &        H &       949.81 &       114.71 \\
sn2005el   &    53693.315 &        H &      1316.87 &       101.68 \\
sn2005el   &    53690.310 &        H &      1374.91 &       109.63 \\
sn2005el   &    53691.295 &        H &      1419.84 &       111.18 \\
sn2005el   &    53689.309 &        H &      1704.06 &        65.56 \\
sn2005el   &    53687.304 &        H &      2020.73 &       115.62 \\
sn2005el   &    53680.351 &        H &      2597.36 &       147.91 \\
sn2005el   &    53678.365 &        H &      3265.76 &       133.15 \\
sn2005el   &    53653.380 &        H &      3317.17 &       139.25 \\
sn2005el   &    53652.362 &        H &      3326.05 &       110.77 \\
sn2005el   &    53654.326 &        H &      3474.31 &       110.48 \\
sn2005el   &    53651.418 &        H &      4020.73 &       120.15 \\
sn2005el   &    53673.274 &        H &      4199.66 &       148.25 \\
sn2005el   &    53667.347 &        H &      4367.61 &       232.70 \\
sn2005el   &    53646.414 &        H &      4639.57 &       149.60 \\
sn2005el   &    53648.379 &        H &      4723.69 &       172.73 \\
sn2005el   &    53663.394 &        H &      4725.20 &       172.64 \\
sn2005el   &    53666.392 &        H &      4823.93 &       156.31 \\
sn2005el   &    53672.290 &        H &      4839.77 &       110.12 \\
sn2005el   &    53665.348 &        H &      4965.73 &       212.43 \\
sn2005el   &    53644.358 &        H &      5303.54 &       129.21 \\
sn2005el   &    53668.327 &        H &      5577.00 &       180.90 \\
sn2005el   &    53643.348 &        H &      5682.60 &       135.74 \\
sn2005el   &    53649.331 &        H &      5734.87 &       566.39 \\
sn2005el   &    53641.349 &        H &      5825.14 &       204.37 \\
sn2005el   &    53642.360 &        H &      5892.09 &       131.22 \\
sn2005el   &    53640.373 &        H &      6029.83 &       181.01 \\
sn2005el   &    53708.293 &        J &       146.87 &        30.53 \\
sn2005el   &    53703.268 &        J &       291.83 &        29.00 \\
sn2005el   &    53703.268 &        J &       295.16 &        29.56 \\
sn2005el   &    53691.295 &        J &       378.50 &        73.80 \\
sn2005el   &    53693.315 &        J &       514.41 &        43.80 \\
sn2005el   &    53689.309 &        J &       688.61 &        43.28 \\
sn2005el   &    53690.313 &        J &       716.13 &        40.41 \\
sn2005el   &    53687.304 &        J &       823.80 &        43.54 \\
sn2005el   &    53680.351 &        J &      1308.44 &        76.92 \\
sn2005el   &    53663.394 &        J &      1440.08 &        61.00 \\
sn2005el   &    53678.365 &        J &      1477.99 &        47.48 \\
sn2005el   &    53665.348 &        J &      1725.10 &        85.55 \\
sn2005el   &    53666.392 &        J &      1779.38 &        55.79 \\
sn2005el   &    53654.326 &        J &      1832.19 &        59.49 \\
sn2005el   &    53667.347 &        J &      1904.91 &        86.41 \\
sn2005el   &    53653.380 &        J &      2168.37 &        74.53 \\
sn2005el   &    53668.327 &        J &      2248.76 &        64.95 \\
sn2005el   &    53673.274 &        J &      2452.56 &        69.58 \\
sn2005el   &    53672.290 &        J &      2558.77 &        43.52 \\
sn2005el   &    53652.363 &        J &      2734.06 &        54.89 \\
sn2005el   &    53651.418 &        J &      3273.90 &        67.36 \\
sn2005el   &    53649.331 &        J &      4420.23 &       220.71 \\
sn2005el   &    53648.379 &        J &      5094.07 &       101.56 \\
sn2005el   &    53646.414 &        J &      5774.23 &        63.44 \\
sn2005el   &    53640.373 &        J &      5955.59 &       102.77 \\
sn2005el   &    53641.349 &        J &      6423.12 &       174.19 \\
sn2005el   &    53642.360 &        J &      6525.89 &       112.64 \\
sn2005el   &    53644.358 &        J &      6548.81 &        93.85 \\
sn2005el   &    53643.348 &        J &      6618.67 &        95.13 \\
sn2005el   &    53691.295 &       Ks &       606.46 &       171.35 \\
sn2005el   &    53708.293 &       Ks &       617.36 &        99.31 \\
sn2005el   &    53703.268 &       Ks &       731.16 &       117.80 \\
sn2005el   &    53703.268 &       Ks &       737.99 &       120.03 \\
sn2005el   &    53690.310 &       Ks &      1334.81 &       126.27 \\
sn2005el   &    53693.315 &       Ks &      1459.92 &       142.42 \\
sn2005el   &    53687.304 &       Ks &      1714.87 &       173.75 \\
sn2005el   &    53689.309 &       Ks &      1716.67 &       170.59 \\
sn2005el   &    53680.351 &       Ks &      2862.08 &       133.52 \\
sn2005el   &    53673.274 &       Ks &      3520.71 &       172.18 \\
sn2005el   &    53678.365 &       Ks &      3697.72 &       246.33 \\
sn2005el   &    53654.326 &       Ks &      4024.19 &       169.75 \\
sn2005el   &    53652.362 &       Ks &      4110.62 &       203.27 \\
sn2005el   &    53653.380 &       Ks &      4206.98 &       257.25 \\
sn2005el   &    53672.290 &       Ks &      4224.88 &       142.39 \\
sn2005el   &    53663.394 &       Ks &      4443.46 &       207.53 \\
sn2005el   &    53649.331 &       Ks &      4517.82 &      1276.13 \\
sn2005el   &    53668.327 &       Ks &      4698.05 &       134.87 \\
sn2005el   &    53665.348 &       Ks &      4928.56 &       268.01 \\
sn2005el   &    53666.392 &       Ks &      4930.39 &       210.01 \\
sn2005el   &    53651.418 &       Ks &      5121.39 &       154.12 \\
sn2005el   &    53648.379 &       Ks &      5416.71 &       184.27 \\
sn2005el   &    53667.347 &       Ks &      5500.11 &       300.87 \\
sn2005el   &    53641.349 &       Ks &      5605.40 &       202.29 \\
sn2005el   &    53646.414 &       Ks &      6105.08 &       193.48 \\
sn2005el   &    53644.358 &       Ks &      6935.43 &       201.55 \\
sn2005el   &    53640.373 &       Ks &      6939.55 &       408.71 \\
sn2005el   &    53642.360 &       Ks &      7350.60 &       289.70 \\
sn2005el   &    53643.348 &       Ks &      7517.96 &       238.91 \\
sn2005eq   &    53992.414 &        H &        -5.69 &       400.01 \\
sn2005eq   &    53696.249 &        H &       -65.28 &       428.38 \\
sn2005eq   &    53708.253 &        H &       105.12 &       113.59 \\
sn2005eq   &    53994.397 &        H &       178.23 &       228.10 \\
sn2005eq   &    53705.202 &        H &       543.54 &        81.95 \\
sn2005eq   &    53663.353 &        H &       610.84 &        77.34 \\
sn2005eq   &    53667.285 &        H &       678.67 &        50.74 \\
sn2005eq   &    53711.229 &        H &       681.39 &        47.46 \\
sn2005eq   &    53703.227 &        H &       708.55 &        69.43 \\
sn2005eq   &    53654.305 &        H &       779.92 &        92.23 \\
sn2005eq   &    53665.307 &        H &       802.10 &        48.26 \\
sn2005eq   &    53700.207 &        H &       820.66 &       186.41 \\
sn2005eq   &    53668.285 &        H &       848.27 &        52.58 \\
sn2005eq   &    53682.291 &        H &       932.51 &        70.88 \\
sn2005eq   &    53666.371 &        H &       941.12 &        73.86 \\
sn2005eq   &    53689.284 &        H &       941.24 &        73.82 \\
sn2005eq   &    53990.448 &        H &      -295.13 &       295.06 \\
sn2005eq   &    53691.230 &        H &      1027.01 &        50.85 \\
sn2005eq   &    53681.296 &        H &      1061.94 &       136.97 \\
sn2005eq   &    53690.247 &        H &      1063.70 &        74.22 \\
sn2005eq   &    53687.262 &        H &      1085.56 &        65.78 \\
sn2005eq   &    53673.233 &        H &      1115.63 &        63.19 \\
sn2005eq   &    53651.386 &        H &      1143.62 &        81.23 \\
sn2005eq   &    53686.360 &        H &      1273.42 &       181.80 \\
sn2005eq   &    53680.330 &        H &      1274.05 &        55.68 \\
sn2005eq   &    53656.282 &        H &      1329.06 &        88.84 \\
sn2005eq   &    53652.321 &        H &      1378.96 &        87.47 \\
sn2005eq   &    53648.316 &        H &      1404.35 &        78.81 \\
sn2005eq   &    53684.336 &        H &      1470.71 &        61.85 \\
sn2005eq   &    53683.319 &        H &      1506.40 &       343.38 \\
sn2005eq   &    53653.359 &        H &      1519.52 &       109.17 \\
sn2005eq   &    53995.372 &        J &        36.25 &       125.76 \\
sn2005eq   &    53992.414 &        J &       -39.33 &       164.35 \\
sn2005eq   &    53994.397 &        J &       -50.92 &        94.10 \\
sn2005eq   &    53990.448 &        J &       117.49 &       154.61 \\
sn2005eq   &    53711.228 &        J &       228.32 &        21.28 \\
sn2005eq   &    53708.252 &        J &       320.21 &        22.67 \\
sn2005eq   &    53703.227 &        J &       335.56 &        40.57 \\
sn2005eq   &    53708.252 &        J &       338.85 &        21.47 \\
sn2005eq   &    53667.285 &        J &       450.47 &        25.85 \\
sn2005eq   &    53700.207 &        J &       456.98 &        28.28 \\
sn2005eq   &    53672.265 &        J &       471.08 &        52.83 \\
sn2005eq   &    53668.285 &        J &       503.70 &        26.06 \\
sn2005eq   &    53673.233 &        J &       522.75 &        23.55 \\
sn2005eq   &    53678.340 &        J &       550.56 &        23.62 \\
sn2005eq   &    53666.371 &        J &       626.65 &        44.41 \\
sn2005eq   &    53682.289 &        J &       638.75 &        25.95 \\
sn2005eq   &    53684.336 &        J &       693.47 &        29.24 \\
sn2005eq   &    53683.310 &        J &       693.70 &        49.69 \\
sn2005eq   &    53680.330 &        J &       703.38 &        18.69 \\
sn2005eq   &    53665.307 &        J &       706.46 &        35.33 \\
sn2005eq   &    53681.296 &        J &       719.28 &        72.21 \\
sn2005eq   &    53663.353 &        J &       734.55 &        32.02 \\
sn2005eq   &    53696.249 &        J &       769.55 &       115.85 \\
sn2005eq   &    53686.358 &        J &       780.39 &        31.61 \\
sn2005eq   &    53687.262 &        J &       846.48 &        26.64 \\
sn2005eq   &    53691.230 &        J &       848.86 &        27.28 \\
sn2005eq   &    53690.247 &        J &       883.26 &        37.39 \\
sn2005eq   &    53689.295 &        J &       984.09 &       110.69 \\
sn2005eq   &    53654.305 &        J &      1545.27 &        36.97 \\
sn2005eq   &    53656.282 &        J &      1586.16 &        44.56 \\
sn2005eq   &    53653.359 &        J &      1626.76 &        34.92 \\
sn2005eq   &    53651.386 &        J &      1938.42 &        35.74 \\
sn2005eq   &    53652.321 &        J &      1959.17 &        32.64 \\
sn2005eq   &    53648.316 &        J &      2022.54 &        50.75 \\
sn2005eq   &    53700.207 &       Ks &        26.12 &      1612.85 \\
sn2005eq   &    53992.414 &       Ks &        44.91 &       869.02 \\
sn2005eq   &    53995.372 &       Ks &       226.28 &       996.94 \\
sn2005eq   &    53672.265 &       Ks &       449.67 &       260.92 \\
sn2005eq   &    53708.252 &       Ks &       571.73 &       147.00 \\
sn2005eq   &    53708.252 &       Ks &       576.01 &       159.89 \\
sn2005eq   &    53703.227 &       Ks &       600.79 &       117.33 \\
sn2005eq   &    53711.228 &       Ks &       654.37 &       119.02 \\
sn2005eq   &    53705.202 &       Ks &       828.50 &       573.68 \\
sn2005eq   &    53687.262 &       Ks &       965.24 &       193.69 \\
sn2005eq   &    53994.397 &       Ks &      -225.77 &      1375.78 \\
sn2005eq   &    53990.448 &       Ks &      -533.21 &      1782.27 \\
sn2005eq   &    53691.230 &       Ks &      1250.75 &       131.83 \\
sn2005eq   &    53663.353 &       Ks &      1373.60 &       146.56 \\
sn2005eq   &    53682.289 &       Ks &      1414.51 &       203.55 \\
sn2005eq   &    53673.233 &       Ks &      1416.17 &       126.19 \\
sn2005eq   &    53683.310 &       Ks &      1468.94 &       252.30 \\
sn2005eq   &    53684.336 &       Ks &      1509.39 &       195.07 \\
sn2005eq   &    53686.358 &       Ks &      1616.94 &       131.66 \\
sn2005eq   &    53689.284 &       Ks &      1652.09 &       162.71 \\
sn2005eq   &    53680.330 &       Ks &      1654.70 &       183.37 \\
sn2005eq   &    53654.305 &       Ks &      1733.46 &       154.90 \\
sn2005eq   &    53656.282 &       Ks &      1745.89 &       217.64 \\
sn2005eq   &    53666.371 &       Ks &      1747.94 &       133.24 \\
sn2005eq   &    53667.285 &       Ks &      1750.22 &       151.18 \\
sn2005eq   &    53665.307 &       Ks &      1792.19 &       203.16 \\
sn2005eq   &    53690.247 &       Ks &      1793.64 &       141.82 \\
sn2005eq   &    53668.285 &       Ks &      1800.71 &       191.50 \\
sn2005eq   &    53651.386 &       Ks &      1827.55 &       131.91 \\
sn2005eq   &    53652.321 &       Ks &      1842.25 &       158.99 \\
sn2005eq   &    53648.316 &       Ks &      1843.04 &       192.51 \\
sn2005eq   &    53681.296 &       Ks &      1880.63 &       366.41 \\
sn2005eq   &    53678.340 &       Ks &      2021.96 &       163.42 \\
sn2005eq   &    53653.359 &       Ks &      2497.26 &       259.48 \\
sn2005eu   &    53928.454 &        H &       -13.61 &       308.25 \\
sn2005eu   &    53728.270 &        H &       -43.54 &       183.59 \\
sn2005eu   &    53926.468 &        H &       166.25 &       228.64 \\
sn2005eu   &    53714.286 &        H &       519.61 &        90.82 \\
sn2005eu   &    53673.143 &        H &       587.20 &       168.67 \\
sn2005eu   &    53670.158 &        H &       630.13 &        44.65 \\
sn2005eu   &    53672.134 &        H &       802.03 &       256.67 \\
sn2005eu   &    53699.286 &        H &       898.12 &       254.69 \\
sn2005eu   &    53674.271 &        H &       911.73 &       155.65 \\
sn2005eu   &    53705.245 &        H &       918.97 &        91.82 \\
sn2005eu   &    53677.250 &        H &       948.24 &        30.04 \\
sn2005eu   &    53687.284 &        H &       952.73 &       193.99 \\
sn2005eu   &    53678.299 &        H &       956.41 &       163.08 \\
sn2005eu   &    53655.197 &        H &       959.94 &       184.21 \\
sn2005eu   &    53680.373 &        H &       963.89 &       112.24 \\
sn2005eu   &    53686.401 &        H &       992.98 &       191.84 \\
sn2005eu   &    53938.415 &        H &      -555.39 &       427.65 \\
sn2005eu   &    53656.179 &        H &      1006.12 &       332.47 \\
sn2005eu   &    53690.332 &        H &      1036.06 &        74.52 \\
sn2005eu   &    53696.312 &        H &      1040.11 &       192.97 \\
sn2005eu   &    53682.241 &        H &      1077.88 &       512.87 \\
sn2005eu   &    53663.284 &        H &      1080.04 &       130.13 \\
sn2005eu   &    53675.264 &        H &      1133.87 &       134.74 \\
sn2005eu   &    53665.173 &        H &      1134.14 &       227.54 \\
sn2005eu   &    53688.342 &        H &      1181.72 &       195.84 \\
sn2005eu   &    53681.249 &        H &      1276.83 &       245.83 \\
sn2005eu   &    53695.346 &        H &      1317.76 &       187.25 \\
sn2005eu   &    53928.454 &        J &        18.40 &        89.66 \\
sn2005eu   &    53714.286 &        J &        75.02 &        17.77 \\
sn2005eu   &    53925.460 &        J &       -27.57 &       103.04 \\
sn2005eu   &    53926.468 &        J &       -95.16 &        82.67 \\
sn2005eu   &    53938.415 &        J &       119.05 &        91.46 \\
sn2005eu   &    53677.250 &        J &       126.44 &        74.42 \\
sn2005eu   &    53728.270 &        J &       143.38 &        71.15 \\
sn2005eu   &    53682.241 &        J &       153.53 &       125.32 \\
sn2005eu   &    53675.264 &        J &       163.42 &        65.50 \\
sn2005eu   &    53678.299 &        J &       226.70 &        68.58 \\
sn2005eu   &    53676.261 &        J &       229.03 &       105.75 \\
sn2005eu   &    53674.271 &        J &       232.66 &        69.92 \\
sn2005eu   &    53672.134 &        J &       275.89 &        63.91 \\
sn2005eu   &    53688.342 &        J &       282.47 &       110.86 \\
sn2005eu   &    53686.401 &        J &       297.05 &        75.92 \\
sn2005eu   &    53680.373 &        J &       316.22 &        77.98 \\
sn2005eu   &    53684.358 &        J &       359.52 &        72.42 \\
sn2005eu   &    53691.311 &        J &       388.98 &       106.64 \\
sn2005eu   &    53705.245 &        J &       390.72 &        86.94 \\
sn2005eu   &    53704.247 &        J &       420.48 &        59.88 \\
sn2005eu   &    53690.332 &        J &       420.77 &       106.07 \\
sn2005eu   &    53700.270 &        J &       479.00 &        86.00 \\
sn2005eu   &    53673.143 &        J &       485.51 &        70.97 \\
sn2005eu   &    53681.249 &        J &       519.93 &       122.92 \\
sn2005eu   &    53670.158 &        J &       546.43 &        42.90 \\
sn2005eu   &    53699.286 &        J &       552.05 &        72.67 \\
sn2005eu   &    53696.312 &        J &       623.00 &        85.61 \\
sn2005eu   &    53695.346 &        J &       762.57 &        70.86 \\
sn2005eu   &    53665.173 &        J &       842.36 &        80.35 \\
sn2005eu   &    53663.284 &        J &       979.61 &       135.49 \\
sn2005eu   &    53656.179 &        J &      1257.89 &       129.15 \\
sn2005eu   &    53655.197 &        J &      1541.91 &       125.99 \\
sn2005eu   &    53681.249 &       Ks &       255.42 &      1117.47 \\
sn2005eu   &    53728.270 &       Ks &       468.78 &       235.35 \\
sn2005eu   &    53704.247 &       Ks &       716.34 &       278.91 \\
sn2005eu   &    53700.270 &       Ks &       740.40 &       312.35 \\
sn2005eu   &    53696.312 &       Ks &       895.32 &       402.85 \\
sn2005eu   &    53938.415 &       Ks &       925.27 &       580.57 \\
sn2005eu   &    53928.454 &       Ks &      -219.84 &       770.28 \\
sn2005eu   &    53926.468 &       Ks &      -590.67 &       498.74 \\
sn2005eu   &    53699.286 &       Ks &      1010.86 &       264.24 \\
sn2005eu   &    53714.286 &       Ks &      1062.87 &       323.36 \\
sn2005eu   &    53665.173 &       Ks &      1154.44 &       392.15 \\
sn2005eu   &    53705.245 &       Ks &      1163.30 &       399.43 \\
sn2005eu   &    53691.311 &       Ks &      1196.46 &       400.08 \\
sn2005eu   &    53656.179 &       Ks &      1215.71 &       564.72 \\
sn2005eu   &    53688.342 &       Ks &      1229.77 &       327.26 \\
sn2005eu   &    53678.299 &       Ks &      1239.13 &       272.53 \\
sn2005eu   &    53680.373 &       Ks &      1245.32 &       326.92 \\
sn2005eu   &    53677.250 &       Ks &      1257.76 &       319.32 \\
sn2005eu   &    53672.134 &       Ks &      1279.06 &       377.78 \\
sn2005eu   &    53684.358 &       Ks &      1288.67 &       323.45 \\
sn2005eu   &    53686.401 &       Ks &      1422.38 &       375.11 \\
sn2005eu   &    53687.284 &       Ks &      1510.47 &       341.08 \\
sn2005eu   &    53682.241 &       Ks &      1582.20 &      1180.78 \\
sn2005eu   &    53663.284 &       Ks &      1604.52 &       341.20 \\
sn2005eu   &    53690.332 &       Ks &      1616.39 &       401.25 \\
sn2005eu   &    53676.261 &       Ks &      1623.14 &       578.61 \\
sn2005eu   &    53674.271 &       Ks &      1702.53 &       333.51 \\
sn2005eu   &    53675.264 &       Ks &      1795.93 &       258.87 \\
sn2005eu   &    53695.346 &       Ks &      1829.83 &       311.46 \\
sn2005eu   &    53655.197 &       Ks &      1891.88 &       324.90 \\
sn2005eu   &    53673.143 &       Ks &      2166.36 &       291.83 \\
sn2005eu   &    53670.158 &       Ks &      2198.90 &       434.31 \\
sn2005hk   &    53928.369 &        H &         0.00 &        98.24 \\
sn2005hk   &    53745.161 &        H &      1146.60 &       177.85 \\
sn2005hk   &    53748.162 &        H &      1218.85 &        64.20 \\
sn2005hk   &    53742.165 &        H &      1602.31 &        91.56 \\
sn2005hk   &    53681.133 &        H &      2153.35 &       234.16 \\
sn2005hk   &    53678.079 &        H &      2341.93 &       163.12 \\
sn2005hk   &    53680.198 &        H &      2570.34 &       100.77 \\
sn2005hk   &    53690.143 &        H &      4586.68 &       155.67 \\
sn2005hk   &    53693.173 &        H &      5066.34 &       183.86 \\
sn2005hk   &    53705.077 &        H &      5164.50 &       114.93 \\
sn2005hk   &    53703.101 &        H &      5666.08 &       196.66 \\
sn2005hk   &    53703.101 &        H &      5712.83 &       198.24 \\
sn2005hk   &    53696.089 &        H &      5730.01 &       286.78 \\
sn2005hk   &    53928.369 &        J &        60.86 &        45.87 \\
sn2005hk   &    53925.361 &        J &       -26.40 &        53.36 \\
sn2005hk   &    53926.362 &        J &       -34.45 &        50.75 \\
sn2005hk   &    53745.161 &        J &       704.19 &        55.59 \\
sn2005hk   &    53748.162 &        J &       821.28 &        34.80 \\
sn2005hk   &    53742.165 &        J &       991.08 &        60.31 \\
sn2005hk   &    53678.079 &        J &      2729.09 &       101.27 \\
sn2005hk   &    53679.090 &        J &      3122.06 &        55.69 \\
sn2005hk   &    53680.198 &        J &      3474.06 &        75.10 \\
sn2005hk   &    53681.133 &        J &      3541.74 &       107.80 \\
sn2005hk   &    53682.092 &        J &      3819.81 &       118.86 \\
sn2005hk   &    53690.143 &        J &      3950.29 &       176.63 \\
sn2005hk   &    53696.089 &        J &      4453.98 &       141.28 \\
sn2005hk   &    53705.077 &        J &      4457.96 &        99.57 \\
sn2005hk   &    53700.146 &        J &      4459.78 &       234.75 \\
sn2005hk   &    53691.164 &        J &      4470.46 &       106.93 \\
sn2005hk   &    53703.101 &        J &      4471.33 &       100.19 \\
sn2005hk   &    53703.101 &        J &      4548.50 &       101.99 \\
sn2005hk   &    53693.173 &        J &      4588.54 &       101.01 \\
sn2005hk   &    53688.198 &        J &      4590.12 &       120.53 \\
sn2005hk   &    53689.177 &        J &      4756.71 &       112.84 \\
sn2005hk   &    53748.162 &       Ks &      1271.11 &       132.39 \\
sn2005hk   &    53678.080 &       Ks &      2157.77 &       209.96 \\
sn2005hk   &    53680.198 &       Ks &      3692.55 &       238.28 \\
sn2005hk   &    53681.133 &       Ks &      3734.31 &       302.17 \\
sn2005hk   &    53688.198 &       Ks &      4855.39 &       371.21 \\
sn2005hk   &    53705.077 &       Ks &      5118.78 &       320.73 \\
sn2005hk   &    53690.143 &       Ks &      5304.42 &       259.61 \\
sn2005hk   &    53703.101 &       Ks &      5937.31 &       181.03 \\
sn2005hk   &    53703.101 &       Ks &      5986.24 &       182.54 \\
sn2005hk   &    53691.164 &       Ks &      5999.55 &       449.90 \\
sn2005hk   &    53689.177 &       Ks &      6032.11 &       294.53 \\
sn2005hk   &    53693.173 &       Ks &      6282.69 &       222.83 \\
sn2005hk   &    53696.089 &       Ks &      6403.32 &       296.73 \\
sn2005iq   &    53928.391 &        H &        -7.16 &       259.16 \\
sn2005iq   &    53926.383 &        H &        11.79 &       398.43 \\
sn2005iq   &    53696.110 &        H &       143.62 &       238.02 \\
sn2005iq   &    53703.081 &        H &       197.78 &       189.11 \\
sn2005iq   &    53695.125 &        H &       213.66 &       186.57 \\
sn2005iq   &    53694.121 &        H &       285.47 &       352.01 \\
sn2005iq   &    53925.389 &        H &       289.16 &       324.19 \\
sn2005iq   &    53704.059 &        H &       290.09 &       189.17 \\
sn2005iq   &    53690.185 &        H &       300.49 &       186.78 \\
sn2005iq   &    53699.112 &        H &       328.14 &       181.78 \\
sn2005iq   &    53689.152 &        H &       332.37 &       120.50 \\
sn2005iq   &    53714.071 &        H &       425.47 &       221.87 \\
sn2005iq   &    53693.127 &        H &       593.76 &       183.67 \\
sn2005iq   &    53688.178 &        H &       784.68 &       148.78 \\
sn2005iq   &    53684.184 &        H &       900.38 &       157.73 \\
sn2005iq   &    53938.393 &        H &      -328.74 &       347.72 \\
sn2005iq   &    53925.389 &        J &       -92.61 &        95.13 \\
sn2005iq   &    53938.393 &        J &       105.13 &       101.36 \\
sn2005iq   &    53704.059 &        J &       133.28 &        83.61 \\
sn2005iq   &    53699.112 &        J &       168.09 &        45.30 \\
sn2005iq   &    53703.081 &        J &       278.08 &        64.40 \\
sn2005iq   &    53694.121 &        J &       339.84 &        69.36 \\
sn2005iq   &    53696.110 &        J &       357.06 &        67.17 \\
sn2005iq   &    53695.125 &        J &       371.86 &        69.76 \\
sn2005iq   &    53714.071 &        J &       453.08 &        78.17 \\
sn2005iq   &    53690.185 &        J &       697.89 &        89.90 \\
sn2005iq   &    53689.152 &        J &       766.61 &        73.18 \\
sn2005iq   &    53688.178 &        J &       895.55 &        79.57 \\
sn2005iq   &    53684.184 &        J &      1205.41 &       104.96 \\
sn2005iq   &    53696.110 &       Ks &        39.71 &       434.28 \\
sn2005iq   &    53925.389 &       Ks &        44.94 &       641.93 \\
sn2005iq   &    53699.112 &       Ks &       -18.18 &       287.88 \\
sn2005iq   &    53714.071 &       Ks &       123.62 &       294.36 \\
sn2005iq   &    53704.059 &       Ks &       126.17 &       369.36 \\
sn2005iq   &    53690.185 &       Ks &       133.66 &       314.52 \\
sn2005iq   &    53695.125 &       Ks &       209.45 &       332.93 \\
sn2005iq   &    53928.391 &       Ks &       248.66 &       645.06 \\
sn2005iq   &    53694.121 &       Ks &       309.43 &       378.23 \\
sn2005iq   &    53693.127 &       Ks &       452.00 &       415.07 \\
sn2005iq   &    53703.081 &       Ks &       546.98 &       271.32 \\
sn2005iq   &    53689.152 &       Ks &       580.35 &       288.97 \\
sn2005iq   &    53684.184 &       Ks &       654.27 &       359.78 \\
sn2005iq   &    53688.178 &       Ks &       661.66 &       429.23 \\
sn2005iq   &    53938.393 &       Ks &      -338.10 &       691.71 \\
sn2005ke   &    53761.118 &        H &       930.19 &       373.74 \\
sn2005ke   &    53766.088 &        H &       942.31 &       106.23 \\
sn2005ke   &    53758.094 &        H &      1121.34 &       145.14 \\
sn2005ke   &    53759.107 &        H &      1245.30 &       143.95 \\
sn2005ke   &    53748.105 &        H &      2385.93 &       144.44 \\
sn2005ke   &    53747.151 &        H &      2504.54 &       175.67 \\
sn2005ke   &    53745.105 &        H &      2600.97 &       183.03 \\
sn2005ke   &    53742.151 &        H &      3668.58 &       110.93 \\
sn2005ke   &    53735.150 &        H &      4469.93 &       264.45 \\
sn2005ke   &    53732.150 &        H &      4627.19 &       394.02 \\
sn2005ke   &    53731.162 &        H &      5465.68 &       221.15 \\
sn2005ke   &    53690.289 &        H &      7260.55 &       508.35 \\
sn2005ke   &    53726.213 &        H &      7603.45 &       159.87 \\
sn2005ke   &    53724.255 &        H &      7889.96 &       281.35 \\
sn2005ke   &    53691.260 &        H &     10192.41 &       608.24 \\
sn2005ke   &    53713.186 &        H &     19005.21 &       494.38 \\
sn2005ke   &    53708.272 &        H &     24378.40 &       859.07 \\
sn2005ke   &    53703.248 &        H &     25570.19 &       628.18 \\
sn2005ke   &    53703.248 &        H &     25583.82 &       628.08 \\
sn2005ke   &    53761.118 &        J &         4.92 &       135.10 \\
sn2005ke   &    53766.088 &        J &       194.41 &        71.28 \\
sn2005ke   &    53763.171 &        J &       242.93 &        76.87 \\
sn2005ke   &    53758.094 &        J &       411.56 &        50.35 \\
sn2005ke   &    53759.107 &        J &       474.62 &        83.55 \\
sn2005ke   &    53748.105 &        J &       671.44 &        64.89 \\
sn2005ke   &    53747.151 &        J &       788.22 &        59.48 \\
sn2005ke   &    53745.105 &        J &       856.14 &        65.37 \\
sn2005ke   &    53742.151 &        J &       968.15 &        74.08 \\
sn2005ke   &    53735.150 &        J &      1919.38 &        63.08 \\
sn2005ke   &    53733.144 &        J &      2073.02 &        95.49 \\
sn2005ke   &    53732.150 &        J &      2302.54 &        99.98 \\
sn2005ke   &    53731.162 &        J &      2366.84 &        99.21 \\
sn2005ke   &    53726.213 &        J &      4165.75 &       120.35 \\
sn2005ke   &    53724.255 &        J &      4662.08 &       176.44 \\
sn2005ke   &    53690.289 &        J &      6249.94 &       326.29 \\
sn2005ke   &    53691.260 &        J &      9313.81 &       392.33 \\
sn2005ke   &    53713.186 &        J &     12551.95 &       443.45 \\
sn2005ke   &    53708.272 &        J &     16487.84 &       331.67 \\
sn2005ke   &    53703.248 &        J &     21164.45 &       744.63 \\
sn2005ke   &    53703.248 &        J &     21365.61 &       751.39 \\
sn2005ke   &    53748.105 &       Ks &      1719.31 &       300.48 \\
sn2005ke   &    53745.105 &       Ks &      2326.08 &       206.53 \\
sn2005ke   &    53735.150 &       Ks &      3236.94 &       379.21 \\
sn2005ke   &    53690.289 &       Ks &      3477.23 &      1347.70 \\
sn2005ke   &    53726.213 &       Ks &      6285.67 &       345.74 \\
sn2005ke   &    53724.255 &       Ks &      6968.35 &       223.64 \\
sn2005ke   &    53691.260 &       Ks &     10559.74 &       655.56 \\
sn2005ke   &    53713.186 &       Ks &     17974.22 &       896.04 \\
sn2005ke   &    53708.272 &       Ks &     23695.22 &       356.98 \\
sn2005ke   &    53703.248 &       Ks &     24141.03 &       479.31 \\
sn2005ke   &    53703.248 &       Ks &     24409.21 &       483.39 \\
sn2005ls   &    53764.170 &        H &      2023.86 &       265.30 \\
sn2005ls   &    53760.127 &        H &      2604.36 &       199.33 \\
sn2005ls   &    53762.069 &        H &      2657.22 &       213.91 \\
sn2005ls   &    53758.140 &        H &      2963.46 &       158.60 \\
sn2005ls   &    53759.149 &        H &      2964.69 &       217.90 \\
sn2005ls   &    53757.114 &        H &      3026.89 &       236.97 \\
sn2005ls   &    53731.200 &        H &      3498.34 &       166.16 \\
sn2005ls   &    53726.234 &        H &      3754.45 &       266.56 \\
sn2005ls   &    53734.203 &        H &      3955.88 &       233.76 \\
sn2005ls   &    53733.166 &        H &      3990.67 &       183.10 \\
sn2005ls   &    53742.117 &        H &      4063.57 &       166.47 \\
sn2005ls   &    53748.120 &        H &      4071.30 &       166.59 \\
sn2005ls   &    53747.186 &        H &      4198.53 &       197.23 \\
sn2005ls   &    53735.129 &        H &      4239.72 &       233.91 \\
sn2005ls   &    53745.120 &        H &      4257.33 &       216.44 \\
sn2005ls   &    53741.120 &        H &      4537.08 &       294.48 \\
sn2005ls   &    53764.170 &        J &       862.39 &        91.61 \\
sn2005ls   &    53762.069 &        J &      1063.04 &       125.48 \\
sn2005ls   &    53760.127 &        J &      1224.62 &       132.50 \\
sn2005ls   &    53758.140 &        J &      1297.91 &       143.20 \\
sn2005ls   &    53731.200 &        J &      1299.45 &        71.06 \\
sn2005ls   &    53726.234 &        J &      1303.73 &       100.18 \\
sn2005ls   &    53734.204 &        J &      1305.05 &       113.15 \\
sn2005ls   &    53733.166 &        J &      1323.15 &        90.42 \\
sn2005ls   &    53759.149 &        J &      1352.94 &        95.27 \\
sn2005ls   &    53735.129 &        J &      1389.97 &       405.46 \\
sn2005ls   &    53757.114 &        J &      1429.35 &        76.19 \\
sn2005ls   &    53742.117 &        J &      1632.34 &       102.26 \\
sn2005ls   &    53741.120 &        J &      1634.43 &       127.28 \\
sn2005ls   &    53745.120 &        J &      1936.19 &        92.84 \\
sn2005ls   &    53747.186 &        J &      1977.76 &       111.13 \\
sn2005ls   &    53748.120 &        J &      2050.49 &        97.60 \\
sn2005ls   &    53758.140 &       Ks &      1804.87 &       821.97 \\
sn2005ls   &    53759.149 &       Ks &      2248.25 &       482.85 \\
sn2005ls   &    53762.069 &       Ks &      2309.16 &       613.15 \\
sn2005ls   &    53757.114 &       Ks &      2868.73 &       327.11 \\
sn2005ls   &    53764.170 &       Ks &      3061.83 &       525.27 \\
sn2005ls   &    53748.120 &       Ks &      3673.10 &       359.58 \\
sn2005ls   &    53747.186 &       Ks &      3968.06 &       417.00 \\
sn2005ls   &    53745.120 &       Ks &      3972.48 &       559.23 \\
sn2005ls   &    53731.200 &       Ks &      4019.77 &       471.25 \\
sn2005ls   &    53742.117 &       Ks &      4064.69 &       499.59 \\
sn2005ls   &    53735.129 &       Ks &      4463.30 &       446.57 \\
sn2005ls   &    53726.234 &       Ks &      4607.00 &       617.78 \\
sn2005ls   &    53741.120 &       Ks &      4734.94 &       749.42 \\
sn2005ls   &    53734.203 &       Ks &      4893.87 &       508.11 \\
sn2005na   &    53992.512 &        H &         0.00 &       222.20 \\
sn2005na   &    53837.125 &        H &       -33.20 &       234.65 \\
sn2005na   &    53838.105 &        H &       -73.18 &       346.88 \\
sn2005na   &    53810.177 &        H &       166.92 &       352.02 \\
sn2005na   &    53797.177 &        H &       397.78 &       349.21 \\
sn2005na   &    53793.152 &        H &       442.38 &       160.04 \\
sn2005na   &    53790.227 &        H &       458.06 &       175.42 \\
sn2005na   &    53786.209 &        H &       796.80 &       216.17 \\
sn2005na   &    53778.260 &        H &       830.90 &       389.65 \\
sn2005na   &    53753.230 &        H &       840.66 &       125.09 \\
sn2005na   &    53759.163 &        H &       932.23 &       261.69 \\
sn2005na   &    53761.159 &        H &       934.49 &       616.68 \\
sn2005na   &    53748.141 &        H &       989.34 &       649.53 \\
sn2005na   &    53807.183 &        H &      -346.12 &       840.90 \\
sn2005na   &    53745.140 &        H &      1090.40 &       196.58 \\
sn2005na   &    53779.235 &        H &      1110.44 &       344.08 \\
sn2005na   &    53757.155 &        H &      1132.50 &       214.24 \\
sn2005na   &    53817.160 &        H &      1138.98 &      1258.43 \\
sn2005na   &    53747.200 &        H &      1156.05 &       219.41 \\
sn2005na   &    53783.289 &        H &      1210.36 &       304.05 \\
sn2005na   &    53758.154 &        H &      1261.85 &       282.31 \\
sn2005na   &    53765.196 &        H &      1349.30 &       218.81 \\
sn2005na   &    53768.211 &        H &      1381.16 &       207.12 \\
sn2005na   &    53780.208 &        H &      1420.61 &      1110.78 \\
sn2005na   &    53763.184 &        H &      1433.83 &       206.92 \\
sn2005na   &    53774.218 &        H &      1465.34 &       361.89 \\
sn2005na   &    53772.172 &        H &      1524.76 &       142.11 \\
sn2005na   &    53766.207 &        H &      1543.97 &       413.82 \\
sn2005na   &    53762.129 &        H &      1570.91 &       204.47 \\
sn2005na   &    53764.185 &        H &      1580.83 &       237.47 \\
sn2005na   &    53767.220 &        H &      1634.85 &       249.53 \\
sn2005na   &    53771.175 &        H &      1637.19 &       211.22 \\
sn2005na   &    53837.104 &        H &      2036.40 &      2568.34 \\
sn2005na   &    53776.238 &        H &      2145.95 &      1178.67 \\
sn2005na   &    53992.512 &        J &         0.00 &       234.22 \\
sn2005na   &    53817.160 &        J &        66.00 &       387.01 \\
sn2005na   &    53837.104 &        J &       -93.46 &       824.01 \\
sn2005na   &    53838.105 &        J &       220.74 &       312.37 \\
sn2005na   &    53793.152 &        J &       235.50 &       197.48 \\
sn2005na   &    53837.125 &        J &       295.41 &       170.45 \\
sn2005na   &    53807.183 &        J &       345.28 &       117.73 \\
sn2005na   &    53797.177 &        J &       348.81 &        92.36 \\
sn2005na   &    53810.177 &        J &       351.10 &       130.51 \\
sn2005na   &    53780.208 &        J &       487.89 &       804.20 \\
sn2005na   &    53783.289 &        J &       523.21 &       132.02 \\
sn2005na   &    53790.227 &        J &       532.18 &       101.72 \\
sn2005na   &    53786.209 &        J &       536.20 &        75.72 \\
sn2005na   &    53753.230 &        J &       586.61 &        67.61 \\
sn2005na   &    53757.155 &        J &       657.84 &        74.25 \\
sn2005na   &    53758.154 &        J &       729.57 &        95.01 \\
sn2005na   &    53759.163 &        J &       737.36 &       139.63 \\
sn2005na   &    53762.129 &        J &       805.80 &        92.41 \\
sn2005na   &    53761.159 &        J &       808.53 &       183.79 \\
sn2005na   &    53763.184 &        J &       857.72 &        87.64 \\
sn2005na   &    53778.260 &        J &       885.72 &       201.14 \\
sn2005na   &    53764.185 &        J &       907.64 &       288.81 \\
sn2005na   &    53765.196 &        J &       931.61 &       166.36 \\
sn2005na   &    53779.235 &        J &       967.03 &       156.19 \\
sn2005na   &    53748.141 &        J &      1093.12 &       193.48 \\
sn2005na   &    53766.207 &        J &      1106.64 &        95.22 \\
sn2005na   &    53747.200 &        J &      1155.47 &       151.65 \\
sn2005na   &    53768.211 &        J &      1167.27 &       102.57 \\
sn2005na   &    53767.220 &        J &      1272.50 &       155.23 \\
sn2005na   &    53772.172 &        J &      1279.65 &       124.56 \\
sn2005na   &    53774.218 &        J &      1387.62 &       180.14 \\
sn2005na   &    53771.175 &        J &      1442.70 &       146.44 \\
sn2005na   &    53776.238 &        J &      1491.39 &       843.64 \\
sn2005na   &    53745.140 &        J &      1528.86 &        69.79 \\
sn2005na   &    53992.512 &       Ks &         0.00 &      1298.46 \\
sn2005na   &    53786.209 &       Ks &       265.85 &       788.43 \\
sn2005na   &    53780.208 &       Ks &       400.59 &      3490.88 \\
sn2005na   &    53810.177 &       Ks &       486.87 &       746.72 \\
sn2005na   &    53748.141 &       Ks &       654.91 &      1997.02 \\
sn2005na   &    53797.177 &       Ks &       683.92 &       863.88 \\
sn2005na   &    53838.105 &       Ks &       766.90 &      3025.59 \\
sn2005na   &    53793.152 &       Ks &       843.28 &       550.38 \\
sn2005na   &    53807.183 &       Ks &       905.81 &       794.21 \\
sn2005na   &    53778.260 &       Ks &      -223.48 &      2673.01 \\
sn2005na   &    53837.104 &       Ks &      -308.07 &      2632.13 \\
sn2005na   &    53747.200 &       Ks &      1159.99 &       595.08 \\
sn2005na   &    53790.227 &       Ks &      1176.08 &       608.53 \\
sn2005na   &    53758.154 &       Ks &      1208.90 &       590.48 \\
sn2005na   &    53774.218 &       Ks &      1231.08 &      1803.09 \\
sn2005na   &    53779.235 &       Ks &      1232.01 &      1470.13 \\
sn2005na   &    53757.155 &       Ks &      1544.87 &       498.39 \\
sn2005na   &    53772.172 &       Ks &      1579.27 &       518.34 \\
sn2005na   &    53763.184 &       Ks &      1596.53 &       687.04 \\
sn2005na   &    53745.140 &       Ks &      1669.50 &       437.81 \\
sn2005na   &    53759.163 &       Ks &      1728.69 &       652.31 \\
sn2005na   &    53766.207 &       Ks &      1816.86 &       533.12 \\
sn2005na   &    53765.196 &       Ks &      1823.91 &       279.07 \\
sn2005na   &    53768.211 &       Ks &      1832.38 &       938.85 \\
sn2005na   &    53762.129 &       Ks &      1854.34 &       746.13 \\
sn2005na   &    53753.230 &       Ks &      1898.31 &       467.04 \\
sn2005na   &    53764.185 &       Ks &      1899.56 &      1163.78 \\
sn2005na   &    53767.220 &       Ks &      1975.88 &       483.13 \\
sn2005na   &    53771.175 &       Ks &      2744.25 &      1495.65 \\
sn2005na   &    53776.238 &       Ks &      2772.34 &      2470.28 \\
sn2005na   &    53837.125 &       Ks &     -3422.66 &     14484.87 \\
sn2006D    &    53852.213 &        H &       372.30 &       264.64 \\
sn2006D    &    53846.330 &        H &       576.52 &       152.96 \\
sn2006D    &    53807.287 &        H &      2609.21 &       351.02 \\
sn2006D    &    53803.283 &        H &      3587.36 &       339.75 \\
sn2006D    &    53800.274 &        H &      4085.91 &       254.65 \\
sn2006D    &    53797.319 &        H &      4739.64 &       388.23 \\
sn2006D    &    53791.336 &        H &      6485.38 &       300.24 \\
sn2006D    &    53788.345 &        H &      7727.15 &       338.92 \\
sn2006D    &    53763.399 &        H &     10077.21 &       590.43 \\
sn2006D    &    53768.382 &        H &     10179.78 &       289.06 \\
sn2006D    &    53764.399 &        H &     10271.12 &       310.19 \\
sn2006D    &    53766.404 &        H &     10622.94 &       266.60 \\
sn2006D    &    53767.394 &        H &     10709.89 &       350.91 \\
sn2006D    &    53758.424 &        H &     11436.13 &       359.57 \\
sn2006D    &    53770.495 &        H &     12234.00 &       293.84 \\
sn2006D    &    53779.329 &        H &     12329.36 &       357.72 \\
sn2006D    &    53771.401 &        H &     12519.47 &       264.47 \\
sn2006D    &    53772.384 &        H &     12520.79 &       365.18 \\
sn2006D    &    53762.423 &        H &     12525.21 &       390.84 \\
sn2006D    &    53778.344 &        H &     12696.84 &       326.54 \\
sn2006D    &    53776.464 &        H &     12797.97 &       355.15 \\
sn2006D    &    53757.530 &        H &     13478.15 &       346.09 \\
sn2006D    &    53753.382 &        H &     16346.06 &       407.70 \\
sn2006D    &    53852.213 &        J &       110.36 &       121.55 \\
sn2006D    &    53846.330 &        J &       145.59 &        80.59 \\
sn2006D    &    53851.236 &        J &       211.70 &        89.07 \\
sn2006D    &    53807.287 &        J &       927.16 &       157.24 \\
sn2006D    &    53803.283 &        J &      1199.45 &       166.05 \\
sn2006D    &    53800.274 &        J &      1448.96 &       109.38 \\
sn2006D    &    53797.319 &        J &      1800.14 &       122.77 \\
sn2006D    &    53791.336 &        J &      3088.62 &       165.12 \\
sn2006D    &    53770.495 &        J &      3550.93 &       158.22 \\
sn2006D    &    53771.401 &        J &      3587.45 &       167.87 \\
sn2006D    &    53772.384 &        J &      3648.78 &       165.36 \\
sn2006D    &    53768.382 &        J &      3736.03 &       157.65 \\
sn2006D    &    53788.345 &        J &      4026.40 &       168.54 \\
sn2006D    &    53774.367 &        J &      4104.52 &       196.04 \\
sn2006D    &    53767.394 &        J &      4178.03 &       169.24 \\
sn2006D    &    53776.464 &        J &      4525.89 &       150.58 \\
sn2006D    &    53766.404 &        J &      4638.53 &       160.86 \\
sn2006D    &    53778.344 &        J &      4743.36 &       190.07 \\
sn2006D    &    53779.329 &        J &      4800.73 &       169.42 \\
sn2006D    &    53764.399 &        J &      6286.67 &       187.79 \\
sn2006D    &    53763.399 &        J &      7547.14 &       353.95 \\
sn2006D    &    53762.420 &        J &      9021.51 &       321.56 \\
sn2006D    &    53758.424 &        J &     14671.23 &       329.38 \\
sn2006D    &    53757.530 &        J &     15597.24 &       381.19 \\
sn2006D    &    53753.382 &        J &     18734.94 &       271.07 \\
sn2006D    &    53846.330 &       Ks &       494.96 &       612.02 \\
sn2006D    &    53852.213 &       Ks &       880.13 &       276.82 \\
sn2006D    &    53807.287 &       Ks &      2143.29 &       415.82 \\
sn2006D    &    53803.283 &       Ks &      2512.92 &       396.67 \\
sn2006D    &    53797.319 &       Ks &      2565.26 &       478.22 \\
sn2006D    &    53800.274 &       Ks &      4312.99 &       666.02 \\
sn2006D    &    53791.336 &       Ks &      5832.71 &       339.71 \\
sn2006D    &    53788.345 &       Ks &      6191.83 &       411.58 \\
sn2006D    &    53762.420 &       Ks &      8819.63 &       714.04 \\
sn2006D    &    53768.382 &       Ks &      9285.91 &       323.49 \\
sn2006D    &    53763.399 &       Ks &      9455.64 &       642.56 \\
sn2006D    &    53771.401 &       Ks &      9503.28 &       422.15 \\
sn2006D    &    53766.404 &       Ks &      9651.53 &       389.80 \\
sn2006D    &    53770.495 &       Ks &     10150.72 &       431.06 \\
sn2006D    &    53767.394 &       Ks &     10227.61 &       385.57 \\
sn2006D    &    53779.329 &       Ks &     10334.79 &       527.18 \\
sn2006D    &    53764.399 &       Ks &     10393.89 &       421.39 \\
sn2006D    &    53772.384 &       Ks &     10558.87 &       405.08 \\
sn2006D    &    53758.424 &       Ks &     14040.08 &       506.47 \\
sn2006D    &    53757.530 &       Ks &     14192.89 &       406.11 \\
sn2006D    &    53753.382 &       Ks &     15272.16 &       681.66 \\
sn2006N    &    53844.121 &        H &        42.95 &       625.57 \\
sn2006N    &    54006.505 &        H &       302.61 &       879.35 \\
sn2006N    &    53811.171 &        H &       445.75 &       559.33 \\
sn2006N    &    53807.245 &        H &       738.49 &       886.63 \\
sn2006N    &    54007.500 &        H &      -448.62 &      1070.69 \\
sn2006N    &    53800.157 &        H &      1526.81 &      1198.82 \\
sn2006N    &    53798.156 &        H &      1642.29 &       226.11 \\
sn2006N    &    53790.186 &        H &      1855.65 &       525.33 \\
sn2006N    &    53797.156 &        H &      1873.06 &       653.41 \\
sn2006N    &    53792.170 &        H &      1935.94 &      1297.52 \\
sn2006N    &    53773.144 &        H &      2039.35 &       825.84 \\
sn2006N    &    53791.159 &        H &      2349.99 &       725.77 \\
sn2006N    &    53766.186 &        H &      2908.14 &       933.57 \\
sn2006N    &    53787.177 &        H &      3056.35 &       299.34 \\
sn2006N    &    53788.202 &        H &      3191.31 &      1283.39 \\
sn2006N    &    53786.128 &        H &      3260.16 &       766.33 \\
sn2006N    &    53765.175 &        H &      3364.81 &       700.01 \\
sn2006N    &    53772.131 &        H &      3376.35 &       684.09 \\
sn2006N    &    53768.191 &        H &      3427.94 &       682.11 \\
sn2006N    &    53783.099 &        H &      3808.50 &      1247.80 \\
sn2006N    &    53794.150 &        H &      3948.81 &      1902.80 \\
sn2006N    &    53767.199 &        H &      4137.80 &       985.03 \\
sn2006N    &    53789.165 &        H &      4369.91 &      1036.27 \\
sn2006N    &    53769.231 &        H &      4652.61 &      1781.51 \\
sn2006N    &    54006.505 &        J &       189.48 &       414.72 \\
sn2006N    &    53811.171 &        J &       320.83 &       290.06 \\
sn2006N    &    53800.157 &        J &       517.70 &       758.54 \\
sn2006N    &    53807.245 &        J &       550.92 &       379.71 \\
sn2006N    &    53798.156 &        J &       836.21 &       123.33 \\
sn2006N    &    54007.500 &        J &      -247.09 &       473.59 \\
sn2006N    &    53844.121 &        J &      -402.82 &       477.49 \\
sn2006N    &    53772.131 &        J &      1108.73 &        79.15 \\
sn2006N    &    53792.170 &        J &      1391.30 &       292.25 \\
sn2006N    &    53769.231 &        J &      1440.27 &       533.50 \\
sn2006N    &    53797.156 &        J &      1515.85 &       215.55 \\
sn2006N    &    53768.191 &        J &      1748.95 &       306.43 \\
sn2006N    &    53794.150 &        J &      1991.20 &       816.17 \\
sn2006N    &    53791.159 &        J &      2112.04 &       183.64 \\
sn2006N    &    53787.177 &        J &      2212.13 &       559.68 \\
sn2006N    &    53786.128 &        J &      2459.70 &       359.23 \\
sn2006N    &    53767.199 &        J &      2533.89 &       115.63 \\
sn2006N    &    53766.186 &        J &      2821.60 &       216.20 \\
sn2006N    &    53788.202 &        J &      2886.84 &       383.01 \\
sn2006N    &    53789.165 &        J &      2948.25 &       427.45 \\
sn2006N    &    53783.099 &        J &      3271.55 &       529.02 \\
sn2006N    &    53765.175 &        J &      3445.68 &       339.55 \\
sn2006N    &    53774.281 &        J &     -1542.51 &      2339.23 \\
sn2006N    &    54006.505 &       Ks &       -21.41 &       566.04 \\
sn2006N    &    54007.500 &       Ks &       339.13 &      2252.78 \\
sn2006N    &    53811.171 &       Ks &      1122.81 &       638.77 \\
sn2006N    &    53807.245 &       Ks &      1304.48 &       963.00 \\
sn2006N    &    53797.156 &       Ks &      1601.50 &      1140.48 \\
sn2006N    &    53794.150 &       Ks &      1753.52 &      2720.00 \\
sn2006N    &    53798.156 &       Ks &      1763.64 &       908.43 \\
sn2006N    &    53844.121 &       Ks &      2303.27 &       801.81 \\
sn2006N    &    53800.157 &       Ks &      2340.41 &      1665.88 \\
sn2006N    &    53790.186 &       Ks &      2423.38 &       772.85 \\
sn2006N    &    53791.159 &       Ks &      2560.53 &       779.09 \\
sn2006N    &    53788.202 &       Ks &      2799.67 &       750.72 \\
sn2006N    &    53769.231 &       Ks &      3020.97 &      1082.84 \\
sn2006N    &    53773.144 &       Ks &      3174.47 &       887.65 \\
sn2006N    &    53783.099 &       Ks &      3195.16 &      1189.10 \\
sn2006N    &    53792.170 &       Ks &      3199.58 &      2241.53 \\
sn2006N    &    53786.128 &       Ks &      3216.20 &       857.95 \\
sn2006N    &    53768.191 &       Ks &      3558.37 &       961.56 \\
sn2006N    &    53772.131 &       Ks &      3629.49 &      1511.29 \\
sn2006N    &    53789.165 &       Ks &      3748.50 &      1027.41 \\
sn2006N    &    53766.186 &       Ks &      4028.98 &       731.34 \\
sn2006N    &    53787.177 &       Ks &      4414.48 &      1390.61 \\
sn2006N    &    53777.126 &       Ks &      4799.59 &      1325.48 \\
sn2006N    &    53765.175 &       Ks &      5153.76 &      1493.63 \\
sn2006N    &    53780.159 &       Ks &     -3627.25 &      9276.59 \\
sn2006X    &    53905.138 &        H &      1435.85 &       207.53 \\
sn2006X    &    53900.152 &        H &      1448.93 &       227.54 \\
sn2006X    &    53891.253 &        H &      1698.21 &       424.55 \\
sn2006X    &    53900.165 &        H &      1859.24 &       229.51 \\
sn2006X    &    53902.140 &        H &      1880.77 &       378.48 \\
sn2006X    &    53904.138 &        H &      1989.60 &       141.80 \\
sn2006X    &    53903.136 &        H &      1991.38 &       219.90 \\
sn2006X    &    53901.143 &        H &      2103.21 &       204.09 \\
sn2006X    &    53887.249 &        H &      2802.60 &       180.26 \\
sn2006X    &    53884.174 &        H &      3296.31 &       247.86 \\
sn2006X    &    53878.175 &        H &      4078.33 &       228.55 \\
sn2006X    &    53884.161 &        H &      4226.23 &       368.76 \\
sn2006X    &    53875.172 &        H &      4298.41 &       290.51 \\
sn2006X    &    53878.254 &        H &      4533.64 &       219.14 \\
sn2006X    &    53875.147 &        H &      5771.11 &       410.78 \\
sn2006X    &    53867.161 &        H &      6810.03 &       326.93 \\
sn2006X    &    53867.175 &        H &      6835.44 &       305.42 \\
sn2006X    &    53864.135 &        H &      7200.56 &       395.38 \\
sn2006X    &    53864.149 &        H &      8142.07 &       364.18 \\
sn2006X    &    53861.151 &        H &      8457.84 &       373.45 \\
sn2006X    &    53861.138 &        H &      8919.69 &       384.62 \\
sn2006X    &    53858.151 &        H &      9411.23 &       319.82 \\
sn2006X    &    53858.157 &        H &      9959.34 &       394.27 \\
sn2006X    &    53852.290 &        H &     11905.78 &       459.89 \\
sn2006X    &    53852.276 &        H &     12568.89 &       635.04 \\
sn2006X    &    53849.371 &        H &     13744.81 &       579.83 \\
sn2006X    &    53849.357 &        H &     13898.20 &       634.97 \\
sn2006X    &    53846.274 &        H &     16221.93 &       608.55 \\
sn2006X    &    53844.163 &        H &     16867.49 &       697.38 \\
sn2006X    &    53846.261 &        H &     16921.23 &       636.48 \\
sn2006X    &    53843.184 &        H &     18525.70 &       580.18 \\
sn2006X    &    53844.177 &        H &     18888.26 &       698.78 \\
sn2006X    &    53841.191 &        H &     18957.33 &       736.35 \\
sn2006X    &    53840.281 &        H &     19449.40 &       487.30 \\
sn2006X    &    53840.294 &        H &     20169.26 &       506.96 \\
sn2006X    &    53837.153 &        H &     22722.30 &      1121.97 \\
sn2006X    &    53837.167 &        H &     23102.42 &       931.16 \\
sn2006X    &    53833.304 &        H &     25110.12 &      1245.84 \\
sn2006X    &    53833.317 &        H &     25350.46 &      1203.62 \\
sn2006X    &    53831.219 &        H &     28418.38 &       532.10 \\
sn2006X    &    53831.205 &        H &     28786.19 &       539.75 \\
sn2006X    &    53825.350 &        H &     33846.03 &      1174.45 \\
sn2006X    &    53825.337 &        H &     37766.42 &      1495.11 \\
sn2006X    &    53820.297 &        H &     45280.72 &      1253.09 \\
sn2006X    &    53797.236 &        H &     47881.34 &      1803.05 \\
sn2006X    &    53794.212 &        H &     51002.75 &      1594.81 \\
sn2006X    &    53792.232 &        H &     51660.21 &      1498.77 \\
sn2006X    &    53800.247 &        H &     52623.28 &      2230.20 \\
sn2006X    &    53789.257 &        H &     52638.95 &      1454.70 \\
sn2006X    &    53798.219 &        H &     53168.61 &      2325.54 \\
sn2006X    &    53791.221 &        H &     54099.76 &      1384.55 \\
sn2006X    &    53787.254 &        H &     54310.16 &      1389.87 \\
sn2006X    &    53788.254 &        H &     55930.94 &      1268.57 \\
sn2006X    &    53799.241 &        H &     56022.08 &      3457.91 \\
sn2006X    &    53790.248 &        H &     56335.32 &      3208.81 \\
sn2006X    &    53786.261 &        H &     57127.11 &      1682.16 \\
sn2006X    &    53802.264 &        H &     57383.27 &      1248.65 \\
sn2006X    &    53808.234 &        H &     57624.37 &      3241.93 \\
sn2006X    &    53785.327 &        H &     57879.31 &      1555.99 \\
sn2006X    &    53803.248 &        H &     60575.18 &       917.32 \\
sn2006X    &    53783.251 &        H &     61066.36 &      3730.17 \\
sn2006X    &    53782.249 &        H &     63314.57 &      1930.40 \\
sn2006X    &    53779.276 &        H &     63566.90 &      1345.81 \\
sn2006X    &    53811.191 &        H &     66733.11 &      1797.33 \\
sn2006X    &    53810.226 &        H &     67236.27 &      4350.17 \\
sn2006X    &    53807.216 &        H &     68147.51 &      1506.88 \\
sn2006X    &    53902.140 &        J &        85.14 &       128.25 \\
sn2006X    &    53900.165 &        J &       103.77 &        98.75 \\
sn2006X    &    53900.152 &        J &       125.89 &        88.27 \\
sn2006X    &    53904.138 &        J &       253.67 &        76.03 \\
sn2006X    &    53901.143 &        J &       365.15 &       132.46 \\
sn2006X    &    53903.136 &        J &       484.22 &        96.87 \\
sn2006X    &    53887.249 &        J &       522.51 &        65.53 \\
sn2006X    &    53905.138 &        J &       586.61 &       127.02 \\
sn2006X    &    53891.253 &        J &       657.73 &       210.36 \\
sn2006X    &    53878.175 &        J &       690.24 &        84.22 \\
sn2006X    &    53878.254 &        J &       747.19 &        57.52 \\
sn2006X    &    53875.172 &        J &       798.06 &        73.86 \\
sn2006X    &    53875.147 &        J &       961.82 &        71.02 \\
sn2006X    &    53887.143 &        J &      -331.44 &       246.12 \\
sn2006X    &    53867.161 &        J &      1198.00 &        80.33 \\
sn2006X    &    53867.175 &        J &      1236.16 &        79.63 \\
sn2006X    &    53864.135 &        J &      1359.51 &       100.88 \\
sn2006X    &    53864.149 &        J &      1504.45 &       116.22 \\
sn2006X    &    53861.151 &        J &      1709.81 &        91.97 \\
sn2006X    &    53861.138 &        J &      1719.20 &        97.48 \\
sn2006X    &    53858.157 &        J &      2059.52 &        92.64 \\
sn2006X    &    53858.151 &        J &      2217.65 &        97.72 \\
sn2006X    &    53852.290 &        J &      2795.32 &       130.78 \\
sn2006X    &    53852.276 &        J &      2798.28 &       115.16 \\
sn2006X    &    53849.371 &        J &      3394.99 &       188.59 \\
sn2006X    &    53846.261 &        J &      4162.91 &       239.99 \\
sn2006X    &    53846.274 &        J &      4618.14 &       193.18 \\
sn2006X    &    53844.177 &        J &      4783.68 &       238.67 \\
sn2006X    &    53843.184 &        J &      5102.17 &       187.69 \\
sn2006X    &    53844.163 &        J &      5125.56 &       174.29 \\
sn2006X    &    53840.281 &        J &      5822.96 &       168.26 \\
sn2006X    &    53841.191 &        J &      5853.36 &       195.69 \\
sn2006X    &    53840.294 &        J &      5923.81 &       171.77 \\
sn2006X    &    53884.161 &        J &      6463.90 &      1225.18 \\
sn2006X    &    53837.167 &        J &      7490.95 &       604.29 \\
sn2006X    &    53837.153 &        J &      7917.56 &       438.25 \\
sn2006X    &    53833.317 &        J &      9530.94 &       457.79 \\
sn2006X    &    53833.304 &        J &      9680.35 &       490.57 \\
sn2006X    &    53831.205 &        J &     10684.94 &       310.42 \\
sn2006X    &    53831.219 &        J &     10757.88 &       266.85 \\
sn2006X    &    53827.435 &        J &     13913.91 &       781.97 \\
sn2006X    &    53799.241 &        J &     15202.71 &      1055.61 \\
sn2006X    &    53800.247 &        J &     15613.65 &       764.54 \\
sn2006X    &    53797.236 &        J &     16069.40 &       748.47 \\
sn2006X    &    53825.337 &        J &     16302.79 &       909.48 \\
sn2006X    &    53798.218 &        J &     16542.72 &       549.51 \\
sn2006X    &    53802.264 &        J &     16594.96 &       434.53 \\
sn2006X    &    53803.248 &        J &     16776.54 &       342.76 \\
sn2006X    &    53825.350 &        J &     16963.76 &       582.62 \\
sn2006X    &    53808.235 &        J &     20157.32 &       953.10 \\
sn2006X    &    53807.216 &        J &     22099.83 &       624.43 \\
sn2006X    &    53794.212 &        J &     23431.00 &       918.26 \\
sn2006X    &    53820.298 &        J &     25457.89 &       703.88 \\
sn2006X    &    53810.226 &        J &     25746.71 &       980.18 \\
sn2006X    &    53811.191 &        J &     29144.06 &       914.96 \\
sn2006X    &    53792.232 &        J &     34675.01 &      1090.09 \\
sn2006X    &    53791.221 &        J &     38332.46 &      1462.83 \\
sn2006X    &    53790.248 &        J &     39495.38 &      2802.84 \\
sn2006X    &    53789.257 &        J &     46906.96 &      1279.66 \\
sn2006X    &    53788.254 &        J &     48494.32 &      1767.85 \\
sn2006X    &    53786.262 &        J &     55871.53 &      3509.33 \\
sn2006X    &    53779.276 &        J &     60734.43 &      1701.16 \\
sn2006X    &    53785.327 &        J &     61365.43 &      2041.84 \\
sn2006X    &    53783.251 &        J &     63138.71 &      5591.93 \\
sn2006X    &    53782.249 &        J &     72049.02 &      2029.05 \\
sn2006X    &    53903.136 &       Ks &      2743.34 &       447.53 \\
sn2006X    &    53887.249 &       Ks &      4329.56 &       315.94 \\
sn2006X    &    53878.254 &       Ks &      4388.06 &       371.39 \\
sn2006X    &    53878.175 &       Ks &      5026.27 &       392.91 \\
sn2006X    &    53875.172 &       Ks &      5604.19 &       444.64 \\
sn2006X    &    53867.161 &       Ks &      8342.59 &       450.17 \\
sn2006X    &    53861.151 &       Ks &      8468.48 &       376.06 \\
sn2006X    &    53861.138 &       Ks &      9412.68 &       319.38 \\
sn2006X    &    53858.157 &       Ks &      9476.07 &       554.06 \\
sn2006X    &    53858.151 &       Ks &      9489.20 &       838.41 \\
sn2006X    &    53840.281 &       Ks &     10170.67 &       851.28 \\
sn2006X    &    53852.276 &       Ks &     11769.21 &       602.56 \\
sn2006X    &    53852.290 &       Ks &     11958.64 &       508.55 \\
sn2006X    &    53849.371 &       Ks &     13138.20 &       489.47 \\
sn2006X    &    53846.274 &       Ks &     16040.15 &       643.83 \\
sn2006X    &    53844.177 &       Ks &     16482.42 &       600.09 \\
sn2006X    &    53843.184 &       Ks &     17618.81 &       494.87 \\
sn2006X    &    53844.163 &       Ks &     17648.29 &       510.71 \\
sn2006X    &    53846.261 &       Ks &     17844.64 &      1024.62 \\
sn2006X    &    53837.153 &       Ks &     18346.85 &      1104.73 \\
sn2006X    &    53837.167 &       Ks &     20531.52 &       812.32 \\
sn2006X    &    53833.317 &       Ks &     24652.80 &      1041.13 \\
sn2006X    &    53831.219 &       Ks &     25600.87 &       682.79 \\
sn2006X    &    53833.304 &       Ks &     25697.49 &      1119.20 \\
sn2006X    &    53831.205 &       Ks &     26456.57 &       663.35 \\
sn2006X    &    53792.232 &       Ks &     30361.19 &      5080.36 \\
sn2006X    &    53825.350 &       Ks &     31016.53 &       926.54 \\
sn2006X    &    53825.337 &       Ks &     35149.92 &       950.45 \\
sn2006X    &    53820.298 &       Ks &     40122.20 &      1111.98 \\
sn2006X    &    53799.241 &       Ks &     50076.04 &      3859.67 \\
sn2006X    &    53797.236 &       Ks &     58010.98 &      2550.66 \\
sn2006X    &    53794.212 &       Ks &     60998.84 &      2346.36 \\
sn2006X    &    53808.235 &       Ks &     63654.49 &      3659.92 \\
sn2006X    &    53791.221 &       Ks &     64085.85 &      2314.70 \\
sn2006X    &    53803.248 &       Ks &     64574.32 &      1306.98 \\
sn2006X    &    53789.257 &       Ks &     65594.89 &      2768.81 \\
sn2006X    &    53802.264 &       Ks &     66974.39 &      1498.77 \\
sn2006X    &    53790.248 &       Ks &     67166.19 &      2380.17 \\
sn2006X    &    53800.247 &       Ks &     67414.68 &      2407.56 \\
sn2006X    &    53788.254 &       Ks &     70326.89 &      2282.78 \\
sn2006X    &    53807.216 &       Ks &     70434.07 &      2148.33 \\
sn2006X    &    53786.262 &       Ks &     74138.65 &      2193.01 \\
sn2006X    &    53811.191 &       Ks &     74941.95 &      1640.17 \\
sn2006X    &    53782.249 &       Ks &     76841.34 &      1558.72 \\
sn2006X    &    53783.251 &       Ks &     78269.35 &      3006.30 \\
sn2006X    &    53785.327 &       Ks &     78532.89 &      2345.95 \\
sn2006X    &    53810.226 &       Ks &     80445.99 &      3234.98 \\
sn2006ac   &    54154.537 &        H &       149.50 &       566.34 \\
sn2006ac   &    53833.208 &        H &       231.34 &       322.23 \\
sn2006ac   &    54157.474 &        H &       351.45 &       418.03 \\
sn2006ac   &    53827.214 &        H &       374.85 &       403.17 \\
sn2006ac   &    53834.244 &        H &       393.56 &       364.82 \\
sn2006ac   &    53839.181 &        H &       401.22 &       279.66 \\
sn2006ac   &    53845.237 &        H &       405.11 &       369.17 \\
sn2006ac   &    53837.202 &        H &       408.30 &       304.46 \\
sn2006ac   &    54158.313 &        H &       482.41 &       380.10 \\
sn2006ac   &    53841.254 &        H &       496.16 &       330.91 \\
sn2006ac   &    53831.255 &        H &       584.44 &       606.64 \\
sn2006ac   &    53825.299 &        H &       600.48 &       357.08 \\
sn2006ac   &    53829.256 &        H &       635.20 &       390.62 \\
sn2006ac   &    53846.227 &        H &       659.87 &       354.64 \\
sn2006ac   &    53842.278 &        H &       686.55 &       395.49 \\
sn2006ac   &    53832.239 &        H &       730.08 &       440.38 \\
sn2006ac   &    53838.176 &        H &       894.58 &       381.77 \\
sn2006ac   &    53818.238 &        H &      1038.59 &       528.43 \\
sn2006ac   &    53817.224 &        H &      1164.75 &       499.73 \\
sn2006ac   &    53794.227 &        H &      1238.58 &       332.01 \\
sn2006ac   &    53790.262 &        H &      1321.52 &       351.68 \\
sn2006ac   &    53798.239 &        H &      1332.19 &       322.44 \\
sn2006ac   &    53783.273 &        H &      1347.42 &       302.34 \\
sn2006ac   &    53792.246 &        H &      1380.02 &       384.52 \\
sn2006ac   &    53823.262 &        H &      1383.58 &       382.21 \\
sn2006ac   &    53799.256 &        H &      1417.08 &       354.33 \\
sn2006ac   &    53787.267 &        H &      1458.49 &       346.28 \\
sn2006ac   &    53811.206 &        H &      1462.53 &       376.23 \\
sn2006ac   &    53800.262 &        H &      1494.02 &       371.54 \\
sn2006ac   &    53782.271 &        H &      1548.58 &       487.07 \\
sn2006ac   &    53802.272 &        H &      1597.43 &       449.18 \\
sn2006ac   &    53820.263 &        H &      1626.89 &       428.26 \\
sn2006ac   &    53786.276 &        H &      1647.13 &       336.62 \\
sn2006ac   &    53797.251 &        H &      1650.55 &       349.88 \\
sn2006ac   &    53791.235 &        H &      1691.67 &       431.10 \\
sn2006ac   &    53810.240 &        H &      1749.96 &       326.74 \\
sn2006ac   &    53788.268 &        H &      1751.34 &       441.24 \\
sn2006ac   &    53781.281 &        H &      1786.97 &       389.78 \\
sn2006ac   &    53808.263 &        H &      1879.73 &       374.14 \\
sn2006ac   &    53803.270 &        H &      2003.40 &       484.74 \\
sn2006ac   &    53807.231 &        H &      2291.75 &       415.20 \\
sn2006ac   &    53833.208 &        J &       258.93 &       203.98 \\
sn2006ac   &    53845.237 &        J &       264.51 &       244.80 \\
sn2006ac   &    54157.474 &        J &       302.14 &       221.27 \\
sn2006ac   &    53834.243 &        J &       316.97 &       213.15 \\
sn2006ac   &    53820.263 &        J &       320.53 &       251.00 \\
sn2006ac   &    53837.202 &        J &       328.85 &       201.55 \\
sn2006ac   &    53841.254 &        J &       354.40 &       206.96 \\
sn2006ac   &    53842.278 &        J &       357.63 &       216.47 \\
sn2006ac   &    53823.262 &        J &       381.07 &       225.58 \\
sn2006ac   &    54158.313 &        J &       403.93 &       213.26 \\
sn2006ac   &    54154.537 &        J &       421.58 &       313.95 \\
sn2006ac   &    53846.227 &        J &       423.77 &       257.91 \\
sn2006ac   &    53831.256 &        J &       450.99 &       443.07 \\
sn2006ac   &    53839.182 &        J &       490.56 &       221.63 \\
sn2006ac   &    53832.239 &        J &       497.43 &       221.12 \\
sn2006ac   &    53838.175 &        J &       530.15 &       278.47 \\
sn2006ac   &    53825.299 &        J &       548.77 &       199.95 \\
sn2006ac   &    53827.213 &        J &       598.39 &       214.04 \\
sn2006ac   &    53797.250 &        J &       642.89 &       178.73 \\
sn2006ac   &    53817.223 &        J &       658.63 &       280.03 \\
sn2006ac   &    53818.235 &        J &       716.44 &       283.45 \\
sn2006ac   &    53790.262 &        J &       717.35 &       193.52 \\
sn2006ac   &    53798.239 &        J &       755.36 &       195.82 \\
sn2006ac   &    53794.227 &        J &       773.75 &       204.11 \\
sn2006ac   &    53792.246 &        J &       775.97 &       204.72 \\
sn2006ac   &    53800.261 &        J &       797.89 &       194.75 \\
sn2006ac   &    53791.235 &        J &       823.21 &       245.69 \\
sn2006ac   &    53829.256 &        J &       833.85 &       231.75 \\
sn2006ac   &    53802.272 &        J &      1078.81 &       251.28 \\
sn2006ac   &    53803.270 &        J &      1083.66 &       260.68 \\
sn2006ac   &    53788.269 &        J &      1088.68 &       255.37 \\
sn2006ac   &    53810.240 &        J &      1204.82 &       207.61 \\
sn2006ac   &    53811.205 &        J &      1226.36 &       213.86 \\
sn2006ac   &    53807.232 &        J &      1241.15 &       246.38 \\
sn2006ac   &    53787.267 &        J &      1314.31 &       196.07 \\
sn2006ac   &    53808.263 &        J &      1346.05 &       210.27 \\
sn2006ac   &    53786.276 &        J &      1598.29 &       209.51 \\
sn2006ac   &    53783.272 &        J &      1762.62 &       209.15 \\
sn2006ac   &    53782.270 &        J &      2114.73 &       270.72 \\
sn2006ac   &    53781.281 &        J &      2252.74 &       278.89 \\
sn2006ac   &    53839.180 &       Ks &        47.22 &       611.92 \\
sn2006ac   &    54158.313 &       Ks &       257.22 &       495.11 \\
sn2006ac   &    53845.237 &       Ks &       270.62 &       491.66 \\
sn2006ac   &    53834.243 &       Ks &       270.85 &       391.28 \\
sn2006ac   &    53842.278 &       Ks &       358.15 &       481.66 \\
sn2006ac   &    54157.474 &       Ks &       505.41 &       554.68 \\
sn2006ac   &    53841.255 &       Ks &       832.14 &       412.55 \\
sn2006ac   &    54154.537 &       Ks &       868.58 &       763.25 \\
sn2006ac   &    53802.273 &       Ks &       909.87 &       381.81 \\
sn2006ac   &    53832.239 &       Ks &       953.61 &       444.71 \\
sn2006ac   &    53823.261 &       Ks &      -363.05 &       948.97 \\
sn2006ac   &    53833.207 &       Ks &      -553.90 &       610.80 \\
sn2006ac   &    53831.255 &       Ks &      -802.43 &      1392.81 \\
sn2006ac   &    53825.301 &       Ks &      1039.56 &       450.51 \\
sn2006ac   &    53794.227 &       Ks &      1297.28 &       454.89 \\
sn2006ac   &    53817.224 &       Ks &      1315.77 &       545.37 \\
sn2006ac   &    53811.205 &       Ks &      1316.89 &       444.66 \\
sn2006ac   &    53803.270 &       Ks &      1371.75 &       662.26 \\
sn2006ac   &    53827.213 &       Ks &      1394.00 &       444.54 \\
sn2006ac   &    53790.263 &       Ks &      1453.08 &       401.99 \\
sn2006ac   &    53800.262 &       Ks &      1469.58 &       401.01 \\
sn2006ac   &    53792.247 &       Ks &      1603.90 &       514.29 \\
sn2006ac   &    53820.263 &       Ks &      1680.33 &       586.55 \\
sn2006ac   &    53838.175 &       Ks &      1778.95 &       565.71 \\
sn2006ac   &    53810.240 &       Ks &      1780.69 &       478.41 \\
sn2006ac   &    53791.235 &       Ks &      1781.27 &       476.34 \\
sn2006ac   &    53788.268 &       Ks &      1864.52 &       504.67 \\
sn2006ac   &    53787.267 &       Ks &      1889.29 &       368.70 \\
sn2006ac   &    53783.272 &       Ks &      1945.67 &       416.11 \\
sn2006ac   &    53797.251 &       Ks &      1978.77 &       506.19 \\
sn2006ac   &    53808.263 &       Ks &      2019.03 &       496.07 \\
sn2006ac   &    53782.272 &       Ks &      2221.07 &       669.93 \\
sn2006ac   &    53807.231 &       Ks &      2223.01 &       574.13 \\
sn2006ac   &    53786.276 &       Ks &      2650.90 &       438.68 \\
sn2006ax   &    54148.362 &        H &         0.00 &       284.26 \\
sn2006ax   &    53818.214 &        H &      1941.25 &       353.00 \\
sn2006ax   &    53838.189 &        H &      2036.04 &       151.30 \\
sn2006ax   &    53817.202 &        H &      2040.26 &       199.58 \\
sn2006ax   &    53837.181 &        H &      2162.50 &       267.57 \\
sn2006ax   &    53834.257 &        H &      2171.95 &       172.94 \\
sn2006ax   &    53864.163 &        H &      2223.08 &       268.29 \\
sn2006ax   &    53863.143 &        H &      2298.86 &       248.03 \\
sn2006ax   &    53831.234 &        H &      2300.11 &       322.13 \\
sn2006ax   &    53827.227 &        H &      2609.78 &       186.11 \\
sn2006ax   &    53860.138 &        H &      2767.43 &       204.87 \\
sn2006ax   &    53832.255 &        H &      2847.35 &       222.47 \\
sn2006ax   &    53850.202 &        H &      3160.03 &       279.18 \\
sn2006ax   &    53825.271 &        H &      3192.98 &       249.66 \\
sn2006ax   &    53859.137 &        H &      3227.78 &       203.38 \\
sn2006ax   &    53820.241 &        H &      3494.20 &       192.11 \\
sn2006ax   &    53851.195 &        H &      3602.36 &       333.52 \\
sn2006ax   &    54148.362 &        J &         0.00 &       138.79 \\
sn2006ax   &    53850.202 &        J &       804.06 &        96.45 \\
sn2006ax   &    53839.194 &        J &       868.49 &        23.46 \\
sn2006ax   &    53838.189 &        J &       995.70 &       120.30 \\
sn2006ax   &    53851.195 &        J &      1223.04 &       135.43 \\
sn2006ax   &    53863.143 &        J &      1224.82 &        57.34 \\
sn2006ax   &    53833.221 &        J &      1247.06 &       295.19 \\
sn2006ax   &    53837.181 &        J &      1298.56 &       197.98 \\
sn2006ax   &    53864.163 &        J &      1313.39 &       151.68 \\
sn2006ax   &    53859.137 &        J &      1640.51 &        82.42 \\
sn2006ax   &    53860.138 &        J &      1692.32 &        58.18 \\
sn2006ax   &    53834.257 &        J &      2145.11 &        68.39 \\
sn2006ax   &    53832.253 &        J &      3016.77 &       105.88 \\
sn2006ax   &    53831.234 &        J &      3100.53 &       103.52 \\
sn2006ax   &    53817.202 &        J &      3136.10 &       201.19 \\
sn2006ax   &    53820.241 &        J &      4322.43 &       149.26 \\
sn2006ax   &    53827.227 &        J &      4534.31 &        63.77 \\
sn2006ax   &    53825.271 &        J &      4899.94 &       242.00 \\
sn2006ax   &    54148.362 &       Ks &         0.00 &       352.37 \\
sn2006ax   &    53833.221 &       Ks &       140.14 &      1161.27 \\
sn2006ax   &    53864.163 &       Ks &      1706.78 &       546.34 \\
sn2006ax   &    53818.214 &       Ks &      1751.62 &       637.46 \\
sn2006ax   &    53817.202 &       Ks &      1752.87 &       229.87 \\
sn2006ax   &    53859.137 &       Ks &      1761.99 &       283.33 \\
sn2006ax   &    53838.189 &       Ks &      1813.04 &       276.92 \\
sn2006ax   &    53850.202 &       Ks &      2103.70 &       522.39 \\
sn2006ax   &    53839.194 &       Ks &      2166.31 &       589.27 \\
sn2006ax   &    53837.181 &       Ks &      2312.00 &       332.81 \\
sn2006ax   &    53863.144 &       Ks &      2448.79 &       412.71 \\
sn2006ax   &    53860.138 &       Ks &      2507.84 &       281.77 \\
sn2006ax   &    53831.234 &       Ks &      2689.48 &       432.70 \\
sn2006ax   &    53832.253 &       Ks &      2903.92 &       220.34 \\
sn2006ax   &    53820.241 &       Ks &      3217.84 &       338.10 \\
sn2006ax   &    53851.195 &       Ks &      3313.43 &       297.49 \\
sn2006ax   &    53834.257 &       Ks &      3339.35 &       340.42 \\
sn2006ax   &    53825.271 &       Ks &      4106.40 &       314.85 \\
sn2006ax   &    53827.227 &       Ks &      4408.88 &       244.10 \\
sn2006cp   &    54161.360 &        H &        -2.54 &        69.74 \\
sn2006cp   &    54162.368 &        H &        -5.69 &        89.88 \\
sn2006cp   &    54161.381 &        H &       -64.79 &        65.49 \\
sn2006cp   &    54162.348 &        H &      -133.16 &        60.24 \\
sn2006cp   &    54162.389 &        H &      -146.74 &       140.36 \\
sn2006cp   &    54161.339 &        H &      -315.11 &        67.36 \\
sn2006cp   &    53904.195 &        H &      1204.66 &        74.68 \\
sn2006cp   &    53905.195 &        H &      1466.12 &        70.92 \\
sn2006cp   &    53900.180 &        H &      1502.23 &       190.07 \\
sn2006cp   &    53902.154 &        H &      1629.69 &        75.74 \\
sn2006cp   &    53901.157 &        H &      1638.63 &       219.78 \\
sn2006cp   &    54162.368 &        J &        -4.79 &        39.20 \\
sn2006cp   &    54161.360 &        J &       -38.48 &        38.98 \\
sn2006cp   &    54161.381 &        J &       -58.17 &        24.08 \\
sn2006cp   &    54161.339 &        J &       -63.67 &        20.48 \\
sn2006cp   &    54162.348 &        J &       -74.53 &        24.43 \\
sn2006cp   &    53905.195 &        J &       739.90 &        33.10 \\
sn2006cp   &    53904.195 &        J &       743.92 &        32.29 \\
sn2006cp   &    54162.389 &        J &      -176.69 &        77.41 \\
sn2006cp   &    53902.154 &        J &      1390.59 &        42.77 \\
sn2006cp   &    53901.157 &        J &      1494.87 &        43.82 \\
sn2006cp   &    53900.180 &        J &      1552.65 &        60.14 \\
sn2006cp   &    54161.381 &       Ks &       150.20 &       104.09 \\
sn2006cp   &    54161.360 &       Ks &      -107.39 &       141.79 \\
sn2006cp   &    54162.368 &       Ks &      -152.31 &       127.99 \\
sn2006cp   &    54161.339 &       Ks &      -206.55 &       122.40 \\
sn2006cp   &    54162.348 &       Ks &      -417.41 &       113.62 \\
sn2006cp   &    54162.389 &       Ks &      -422.59 &       155.66 \\
sn2006cp   &    53900.180 &       Ks &      1589.93 &       783.60 \\
sn2006cp   &    53901.157 &       Ks &      1634.74 &       903.52 \\
sn2006cp   &    53905.195 &       Ks &      1667.69 &       205.44 \\
sn2006cp   &    53902.154 &       Ks &      1774.03 &       163.35 \\
sn2006cp   &    53904.195 &       Ks &      1829.25 &       213.47 \\
sn2006cz   &    54161.485 &        H &       -18.26 &       437.39 \\
sn2006cz   &    54161.444 &        H &       -52.07 &       241.79 \\
sn2006cz   &    54162.445 &        H &       209.62 &       461.07 \\
sn2006cz   &    53904.174 &        H &       294.34 &       207.78 \\
sn2006cz   &    53903.172 &        H &       484.70 &       313.06 \\
sn2006cz   &    53905.174 &        H &       612.83 &       177.37 \\
sn2006cz   &    54162.445 &        J &        94.42 &        99.61 \\
sn2006cz   &    53904.174 &        J &       786.38 &        75.08 \\
sn2006cz   &    53903.172 &        J &       862.67 &       106.03 \\
sn2006cz   &    53905.174 &        J &       898.30 &        76.20 \\
sn2006cz   &    54161.444 &        J &      -141.67 &       122.01 \\
sn2006cz   &    54161.464 &       Ks &        57.91 &       771.11 \\
sn2006cz   &    54161.444 &       Ks &       -45.01 &       370.23 \\
sn2006cz   &    53904.174 &       Ks &       735.38 &       609.43 \\
sn2006cz   &    54162.445 &       Ks &      -499.09 &       569.41 \\
sn2006cz   &    53903.172 &       Ks &      1359.22 &       535.53 \\
sn2006cz   &    54161.485 &       Ks &      1374.99 &       881.31 \\
sn2006cz   &    53905.174 &       Ks &      1434.51 &       781.07 \\
sn2006le   &    54153.148 &        H &        69.58 &       421.55 \\
sn2006le   &    54156.128 &        H &       -58.89 &       430.91 \\
sn2006le   &    54154.143 &        H &       205.98 &       472.18 \\
sn2006le   &    54101.166 &        H &       896.76 &       366.82 \\
sn2006le   &    54157.148 &        H &      -137.36 &       370.95 \\
sn2006le   &    54099.296 &        H &      1039.02 &       202.82 \\
sn2006le   &    54094.198 &        H &      1041.23 &       343.72 \\
sn2006le   &    54093.189 &        H &      1141.52 &       221.94 \\
sn2006le   &    54052.312 &        H &      1331.53 &       305.70 \\
sn2006le   &    54057.275 &        H &      1388.15 &       396.69 \\
sn2006le   &    54063.292 &        H &      1411.37 &       528.56 \\
sn2006le   &    54090.221 &        H &      1496.24 &       280.05 \\
sn2006le   &    54086.193 &        H &      1637.75 &       206.01 \\
sn2006le   &    54060.254 &        H &      1708.01 &        63.00 \\
sn2006le   &    54085.167 &        H &      1751.95 &       332.39 \\
sn2006le   &    54058.211 &        H &      1812.97 &       296.51 \\
sn2006le   &    54061.248 &        H &      1828.11 &        40.86 \\
sn2006le   &    54064.270 &        H &      1928.37 &       299.87 \\
sn2006le   &    54069.201 &        H &      1945.82 &      1547.12 \\
sn2006le   &    54050.306 &        H &      1960.98 &       431.44 \\
sn2006le   &    54049.290 &        H &      2002.13 &       318.58 \\
sn2006le   &    54081.140 &        H &      2018.52 &       131.47 \\
sn2006le   &    54043.355 &        H &      2092.06 &       508.39 \\
sn2006le   &    54066.394 &        H &      2108.74 &       284.14 \\
sn2006le   &    54051.404 &        H &      2185.97 &       416.09 \\
sn2006le   &    54047.281 &        H &      2217.41 &       112.13 \\
sn2006le   &    54071.190 &        H &      2228.01 &       698.85 \\
sn2006le   &    54045.327 &        H &      2230.04 &       173.68 \\
sn2006le   &    54053.322 &        H &      2312.34 &       282.55 \\
sn2006le   &    54070.206 &        H &      2334.06 &       359.07 \\
sn2006le   &    54079.217 &        H &      2397.67 &       354.45 \\
sn2006le   &    54083.173 &        H &      2427.42 &       281.95 \\
sn2006le   &    54074.186 &        H &      2452.88 &       273.61 \\
sn2006le   &    54042.357 &        H &      2478.67 &       361.26 \\
sn2006le   &    54080.145 &        H &      2480.47 &       228.63 \\
sn2006le   &    54072.193 &        H &      2557.58 &       290.14 \\
sn2006le   &    54044.326 &        H &      2585.91 &       358.59 \\
sn2006le   &    54041.353 &        H &      2752.62 &       244.12 \\
sn2006le   &    54077.157 &        H &      2813.90 &       130.32 \\
sn2006le   &    54157.147 &        J &        15.36 &       129.38 \\
sn2006le   &    54154.143 &        J &       -14.15 &       116.11 \\
sn2006le   &    54156.128 &        J &       100.55 &       133.02 \\
sn2006le   &    54100.170 &        J &       419.30 &        58.15 \\
sn2006le   &    54095.141 &        J &       442.64 &       116.93 \\
sn2006le   &    54096.147 &        J &       455.92 &       200.49 \\
sn2006le   &    54101.166 &        J &       521.48 &       127.62 \\
sn2006le   &    54061.248 &        J &       598.14 &       101.06 \\
sn2006le   &    54064.270 &        J &       601.03 &       153.00 \\
sn2006le   &    54066.394 &        J &       603.98 &        93.38 \\
sn2006le   &    54063.292 &        J &       611.15 &       134.31 \\
sn2006le   &    54093.189 &        J &       634.37 &        86.18 \\
sn2006le   &    54060.254 &        J &       672.57 &       143.02 \\
sn2006le   &    54071.190 &        J &       680.87 &       164.45 \\
sn2006le   &    54094.198 &        J &       696.47 &       125.06 \\
sn2006le   &    54091.218 &        J &       713.79 &        84.10 \\
sn2006le   &    54070.206 &        J &       743.85 &        88.03 \\
sn2006le   &    54074.186 &        J &       840.61 &        85.57 \\
sn2006le   &    54072.193 &        J &       946.78 &       115.31 \\
sn2006le   &    54153.148 &        J &      -134.85 &       155.88 \\
sn2006le   &    54076.156 &        J &      1055.33 &       122.39 \\
sn2006le   &    54058.211 &        J &      1097.22 &       221.09 \\
sn2006le   &    54086.193 &        J &      1132.24 &        93.23 \\
sn2006le   &    54085.167 &        J &      1133.73 &       148.18 \\
sn2006le   &    54080.145 &        J &      1159.89 &       132.00 \\
sn2006le   &    54077.157 &        J &      1170.73 &       223.19 \\
sn2006le   &    54079.217 &        J &      1192.39 &       159.31 \\
sn2006le   &    54078.320 &        J &      1238.46 &       167.24 \\
sn2006le   &    54084.177 &        J &      1331.42 &       122.12 \\
sn2006le   &    54056.279 &        J &      1360.94 &       144.83 \\
sn2006le   &    54081.140 &        J &      1444.88 &       110.13 \\
sn2006le   &    54055.395 &        J &      1548.74 &       210.98 \\
sn2006le   &    54052.312 &        J &      1928.92 &       284.46 \\
sn2006le   &    54053.322 &        J &      1938.38 &       187.21 \\
sn2006le   &    54051.404 &        J &      2334.90 &       129.42 \\
sn2006le   &    54050.306 &        J &      2680.97 &       249.80 \\
sn2006le   &    54049.290 &        J &      2862.75 &       242.05 \\
sn2006le   &    54048.290 &        J &      2894.55 &       207.56 \\
sn2006le   &    54047.281 &        J &      2984.45 &       288.30 \\
sn2006le   &    54040.346 &        J &      3075.03 &       223.63 \\
sn2006le   &    54045.327 &        J &      3290.65 &       412.29 \\
sn2006le   &    54044.326 &        J &      3438.76 &       226.55 \\
sn2006le   &    54041.353 &        J &      3460.40 &       316.44 \\
sn2006le   &    54154.143 &       Ks &        37.99 &       668.21 \\
sn2006le   &    54153.148 &       Ks &        61.12 &       491.50 \\
sn2006le   &    54101.166 &       Ks &       319.44 &       630.15 \\
sn2006le   &    54156.128 &       Ks &       393.46 &       615.98 \\
sn2006le   &    54100.170 &       Ks &       533.12 &       371.24 \\
sn2006le   &    54094.198 &       Ks &       627.88 &       400.03 \\
sn2006le   &    54096.147 &       Ks &       647.27 &       194.35 \\
sn2006le   &    54157.147 &       Ks &      -266.94 &       440.60 \\
sn2006le   &    54090.221 &       Ks &      1021.70 &       485.97 \\
sn2006le   &    54091.218 &       Ks &      1223.74 &       433.33 \\
sn2006le   &    54099.296 &       Ks &      1267.49 &      1544.48 \\
sn2006le   &    54095.141 &       Ks &      1507.63 &       470.56 \\
sn2006le   &    54083.173 &       Ks &      1721.42 &       463.49 \\
sn2006le   &    54093.189 &       Ks &      1747.28 &       307.26 \\
sn2006le   &    54086.193 &       Ks &      1821.77 &       505.59 \\
sn2006le   &    54085.167 &       Ks &      1897.34 &       582.94 \\
sn2006le   &    54052.312 &       Ks &      2030.68 &       700.46 \\
sn2006le   &    54063.292 &       Ks &      2039.58 &       423.09 \\
sn2006le   &    54061.248 &       Ks &      2165.00 &       517.70 \\
sn2006le   &    54076.156 &       Ks &      2166.01 &       487.18 \\
sn2006le   &    54050.306 &       Ks &      2230.14 &       722.98 \\
sn2006le   &    54069.201 &       Ks &      2244.01 &      1270.06 \\
sn2006le   &    54081.140 &       Ks &      2283.62 &       523.54 \\
sn2006le   &    54058.211 &       Ks &      2314.51 &       764.76 \\
sn2006le   &    54071.190 &       Ks &      2391.16 &       565.98 \\
sn2006le   &    54080.145 &       Ks &      2396.21 &       525.79 \\
sn2006le   &    54066.394 &       Ks &      2419.03 &       448.08 \\
sn2006le   &    54060.254 &       Ks &      2471.25 &       629.93 \\
sn2006le   &    54079.217 &       Ks &      2487.83 &      1389.61 \\
sn2006le   &    54084.177 &       Ks &      2591.94 &       495.47 \\
sn2006le   &    54074.186 &       Ks &      2602.90 &       488.67 \\
sn2006le   &    54072.193 &       Ks &      2605.18 &       593.25 \\
sn2006le   &    54057.275 &       Ks &      2748.74 &       829.45 \\
sn2006le   &    54064.270 &       Ks &      2754.92 &       323.05 \\
sn2006le   &    54078.320 &       Ks &      2788.60 &       623.28 \\
sn2006le   &    54056.279 &       Ks &      2846.49 &       733.11 \\
sn2006le   &    54053.322 &       Ks &      2922.04 &       600.21 \\
sn2006le   &    54045.327 &       Ks &      2924.48 &       674.06 \\
sn2006le   &    54070.206 &       Ks &      2951.29 &       653.68 \\
sn2006le   &    54051.404 &       Ks &      3014.21 &       554.00 \\
sn2006le   &    54044.326 &       Ks &      3098.10 &       504.68 \\
sn2006le   &    54055.395 &       Ks &      3103.45 &       754.76 \\
sn2006le   &    54047.281 &       Ks &      3116.98 &       724.56 \\
sn2006le   &    54077.157 &       Ks &      3135.58 &       607.67 \\
sn2006le   &    54041.353 &       Ks &      3157.26 &       611.46 \\
sn2006le   &    54042.357 &       Ks &      3159.56 &      1206.46 \\
sn2006le   &    54048.290 &       Ks &      3357.65 &       690.15 \\
sn2006le   &    54040.346 &       Ks &      3381.75 &       311.64 \\
sn2006le   &    54043.355 &       Ks &      3677.64 &      1202.61 \\
sn2006le   &    54049.290 &       Ks &      3800.38 &       595.08 \\
sn2006cp   &    54161.360 &        H &        -2.54 &        69.74 \\
sn2006cp   &    54162.368 &        H &        -5.69 &        89.88 \\
sn2006cp   &    54161.381 &        H &       -64.79 &        65.49 \\
sn2006cp   &    54162.348 &        H &      -133.16 &        60.24 \\
sn2006cp   &    54162.389 &        H &      -146.74 &       140.36 \\
sn2006cp   &    54161.339 &        H &      -315.11 &        67.36 \\
sn2006cp   &    53904.195 &        H &      1204.66 &        74.68 \\
sn2006cp   &    53905.195 &        H &      1466.12 &        70.92 \\
sn2006cp   &    53900.180 &        H &      1502.23 &       190.07 \\
sn2006cp   &    53902.154 &        H &      1629.69 &        75.74 \\
sn2006cp   &    53901.157 &        H &      1638.63 &       219.78 \\
sn2006cp   &    54162.368 &        J &        -4.79 &        39.20 \\
sn2006cp   &    54161.360 &        J &       -38.48 &        38.98 \\
sn2006cp   &    54161.381 &        J &       -58.17 &        24.08 \\
sn2006cp   &    54161.339 &        J &       -63.67 &        20.48 \\
sn2006cp   &    54162.348 &        J &       -74.53 &        24.43 \\
sn2006cp   &    53905.195 &        J &       739.90 &        33.10 \\
sn2006cp   &    53904.195 &        J &       743.92 &        32.29 \\
sn2006cp   &    54162.389 &        J &      -176.69 &        77.41 \\
sn2006cp   &    53902.154 &        J &      1390.59 &        42.77 \\
sn2006cp   &    53901.157 &        J &      1494.87 &        43.82 \\
sn2006cp   &    53900.180 &        J &      1552.65 &        60.14 \\
sn2006cp   &    54161.381 &       Ks &       150.20 &       104.09 \\
sn2006cp   &    54161.360 &       Ks &      -107.39 &       141.79 \\
sn2006cp   &    54162.368 &       Ks &      -152.31 &       127.99 \\
sn2006cp   &    54161.339 &       Ks &      -206.55 &       122.40 \\
sn2006cp   &    54162.348 &       Ks &      -417.41 &       113.62 \\
sn2006cp   &    54162.389 &       Ks &      -422.59 &       155.66 \\
sn2006cp   &    53900.180 &       Ks &      1589.93 &       783.60 \\
sn2006cp   &    53901.157 &       Ks &      1634.74 &       903.52 \\
sn2006cp   &    53905.195 &       Ks &      1667.69 &       205.44 \\
sn2006cp   &    53902.154 &       Ks &      1774.03 &       163.35 \\
sn2006cp   &    53904.195 &       Ks &      1829.25 &       213.47 \\
sn2006gr   &    54004.192 &        H &        98.12 &       132.79 \\
sn2006gr   &    54003.179 &        H &       166.26 &       135.32 \\
sn2006gr   &    54007.185 &        H &       382.22 &       111.27 \\
sn2006gr   &    54005.192 &        H &       538.30 &       164.69 \\
sn2006gr   &    54006.193 &        H &       732.14 &       160.47 \\
sn2006gr   &    54008.184 &        H &       747.83 &       119.91 \\
sn2006gr   &    54003.179 &        J &       304.62 &        43.08 \\
sn2006gr   &    54004.192 &        J &       428.75 &        30.49 \\
sn2006gr   &    54005.192 &        J &       563.95 &        44.82 \\
sn2006gr   &    54006.193 &        J &       583.26 &        39.86 \\
sn2006gr   &    54008.184 &        J &       723.14 &        28.19 \\
sn2006gr   &    54007.185 &        J &       733.08 &        49.99 \\
sn2006gr   &    54008.184 &       Ks &       -15.53 &       199.79 \\
sn2006gr   &    54003.179 &       Ks &       -46.70 &       221.52 \\
sn2006gr   &    54005.192 &       Ks &       -49.71 &       160.98 \\
sn2006gr   &    54007.185 &       Ks &       216.21 &       244.18 \\
sn2006gr   &    54006.193 &       Ks &       630.67 &       245.71 \\
sn2006gr   &    54004.192 &       Ks &       813.54 &       184.88 \\
sn2006le   &    54153.148 &        H &        69.58 &       421.55 \\
sn2006le   &    54156.128 &        H &       -58.89 &       430.91 \\
sn2006le   &    54154.143 &        H &       205.98 &       472.18 \\
sn2006le   &    54101.166 &        H &       896.76 &       366.82 \\
sn2006le   &    54157.148 &        H &      -137.36 &       370.95 \\
sn2006le   &    54099.296 &        H &      1039.02 &       202.82 \\
sn2006le   &    54094.198 &        H &      1041.23 &       343.72 \\
sn2006le   &    54093.189 &        H &      1141.52 &       221.94 \\
sn2006le   &    54052.312 &        H &      1331.53 &       305.70 \\
sn2006le   &    54057.275 &        H &      1388.15 &       396.69 \\
sn2006le   &    54063.292 &        H &      1411.37 &       528.56 \\
sn2006le   &    54090.221 &        H &      1496.24 &       280.05 \\
sn2006le   &    54086.193 &        H &      1637.75 &       206.01 \\
sn2006le   &    54060.254 &        H &      1708.01 &        63.00 \\
sn2006le   &    54085.167 &        H &      1751.95 &       332.39 \\
sn2006le   &    54058.211 &        H &      1812.97 &       296.51 \\
sn2006le   &    54061.248 &        H &      1828.11 &        40.86 \\
sn2006le   &    54064.270 &        H &      1928.37 &       299.87 \\
sn2006le   &    54069.201 &        H &      1945.82 &      1547.12 \\
sn2006le   &    54050.306 &        H &      1960.98 &       431.44 \\
sn2006le   &    54049.290 &        H &      2002.13 &       318.58 \\
sn2006le   &    54081.140 &        H &      2018.52 &       131.47 \\
sn2006le   &    54043.355 &        H &      2092.06 &       508.39 \\
sn2006le   &    54066.394 &        H &      2108.74 &       284.14 \\
sn2006le   &    54051.404 &        H &      2185.97 &       416.09 \\
sn2006le   &    54047.281 &        H &      2217.41 &       112.13 \\
sn2006le   &    54071.190 &        H &      2228.01 &       698.85 \\
sn2006le   &    54045.327 &        H &      2230.04 &       173.68 \\
sn2006le   &    54053.322 &        H &      2312.34 &       282.55 \\
sn2006le   &    54070.206 &        H &      2334.06 &       359.07 \\
sn2006le   &    54079.217 &        H &      2397.67 &       354.45 \\
sn2006le   &    54083.173 &        H &      2427.42 &       281.95 \\
sn2006le   &    54074.186 &        H &      2452.88 &       273.61 \\
sn2006le   &    54042.357 &        H &      2478.67 &       361.26 \\
sn2006le   &    54080.145 &        H &      2480.47 &       228.63 \\
sn2006le   &    54072.193 &        H &      2557.58 &       290.14 \\
sn2006le   &    54044.326 &        H &      2585.91 &       358.59 \\
sn2006le   &    54041.353 &        H &      2752.62 &       244.12 \\
sn2006le   &    54077.157 &        H &      2813.90 &       130.32 \\
sn2006le   &    54157.147 &        J &        15.36 &       129.38 \\
sn2006le   &    54154.143 &        J &       -14.15 &       116.11 \\
sn2006le   &    54156.128 &        J &       100.55 &       133.02 \\
sn2006le   &    54100.170 &        J &       419.30 &        58.15 \\
sn2006le   &    54095.141 &        J &       442.64 &       116.93 \\
sn2006le   &    54096.147 &        J &       455.92 &       200.49 \\
sn2006le   &    54101.166 &        J &       521.48 &       127.62 \\
sn2006le   &    54061.248 &        J &       598.14 &       101.06 \\
sn2006le   &    54064.270 &        J &       601.03 &       153.00 \\
sn2006le   &    54066.394 &        J &       603.98 &        93.38 \\
sn2006le   &    54063.292 &        J &       611.15 &       134.31 \\
sn2006le   &    54093.189 &        J &       634.37 &        86.18 \\
sn2006le   &    54060.254 &        J &       672.57 &       143.02 \\
sn2006le   &    54071.190 &        J &       680.87 &       164.45 \\
sn2006le   &    54094.198 &        J &       696.47 &       125.06 \\
sn2006le   &    54091.218 &        J &       713.79 &        84.10 \\
sn2006le   &    54070.206 &        J &       743.85 &        88.03 \\
sn2006le   &    54074.186 &        J &       840.61 &        85.57 \\
sn2006le   &    54072.193 &        J &       946.78 &       115.31 \\
sn2006le   &    54153.148 &        J &      -134.85 &       155.88 \\
sn2006le   &    54076.156 &        J &      1055.33 &       122.39 \\
sn2006le   &    54058.211 &        J &      1097.22 &       221.09 \\
sn2006le   &    54086.193 &        J &      1132.24 &        93.23 \\
sn2006le   &    54085.167 &        J &      1133.73 &       148.18 \\
sn2006le   &    54080.145 &        J &      1159.89 &       132.00 \\
sn2006le   &    54077.157 &        J &      1170.73 &       223.19 \\
sn2006le   &    54079.217 &        J &      1192.39 &       159.31 \\
sn2006le   &    54078.320 &        J &      1238.46 &       167.24 \\
sn2006le   &    54084.177 &        J &      1331.42 &       122.12 \\
sn2006le   &    54056.279 &        J &      1360.94 &       144.83 \\
sn2006le   &    54081.140 &        J &      1444.88 &       110.13 \\
sn2006le   &    54055.395 &        J &      1548.74 &       210.98 \\
sn2006le   &    54052.312 &        J &      1928.92 &       284.46 \\
sn2006le   &    54053.322 &        J &      1938.38 &       187.21 \\
sn2006le   &    54051.404 &        J &      2334.90 &       129.42 \\
sn2006le   &    54050.306 &        J &      2680.97 &       249.80 \\
sn2006le   &    54049.290 &        J &      2862.75 &       242.05 \\
sn2006le   &    54048.290 &        J &      2894.55 &       207.56 \\
sn2006le   &    54047.281 &        J &      2984.45 &       288.30 \\
sn2006le   &    54040.346 &        J &      3075.03 &       223.63 \\
sn2006le   &    54045.327 &        J &      3290.65 &       412.29 \\
sn2006le   &    54044.326 &        J &      3438.76 &       226.55 \\
sn2006le   &    54041.353 &        J &      3460.40 &       316.44 \\
sn2006le   &    54154.143 &       Ks &        37.99 &       668.21 \\
sn2006le   &    54153.148 &       Ks &        61.12 &       491.50 \\
sn2006le   &    54101.166 &       Ks &       319.44 &       630.15 \\
sn2006le   &    54156.128 &       Ks &       393.46 &       615.98 \\
sn2006le   &    54100.170 &       Ks &       533.12 &       371.24 \\
sn2006le   &    54094.198 &       Ks &       627.88 &       400.03 \\
sn2006le   &    54096.147 &       Ks &       647.27 &       194.35 \\
sn2006le   &    54157.147 &       Ks &      -266.94 &       440.60 \\
sn2006le   &    54090.221 &       Ks &      1021.70 &       485.97 \\
sn2006le   &    54091.218 &       Ks &      1223.74 &       433.33 \\
sn2006le   &    54099.296 &       Ks &      1267.49 &      1544.48 \\
sn2006le   &    54095.141 &       Ks &      1507.63 &       470.56 \\
sn2006le   &    54083.173 &       Ks &      1721.42 &       463.49 \\
sn2006le   &    54093.189 &       Ks &      1747.28 &       307.26 \\
sn2006le   &    54086.193 &       Ks &      1821.77 &       505.59 \\
sn2006le   &    54085.167 &       Ks &      1897.34 &       582.94 \\
sn2006le   &    54052.312 &       Ks &      2030.68 &       700.46 \\
sn2006le   &    54063.292 &       Ks &      2039.58 &       423.09 \\
sn2006le   &    54061.248 &       Ks &      2165.00 &       517.70 \\
sn2006le   &    54076.156 &       Ks &      2166.01 &       487.18 \\
sn2006le   &    54050.306 &       Ks &      2230.14 &       722.98 \\
sn2006le   &    54069.201 &       Ks &      2244.01 &      1270.06 \\
sn2006le   &    54081.140 &       Ks &      2283.62 &       523.54 \\
sn2006le   &    54058.211 &       Ks &      2314.51 &       764.76 \\
sn2006le   &    54071.190 &       Ks &      2391.16 &       565.98 \\
sn2006le   &    54080.145 &       Ks &      2396.21 &       525.79 \\
sn2006le   &    54066.394 &       Ks &      2419.03 &       448.08 \\
sn2006le   &    54060.254 &       Ks &      2471.25 &       629.93 \\
sn2006le   &    54079.217 &       Ks &      2487.83 &      1389.61 \\
sn2006le   &    54084.177 &       Ks &      2591.94 &       495.47 \\
sn2006le   &    54074.186 &       Ks &      2602.90 &       488.67 \\
sn2006le   &    54072.193 &       Ks &      2605.18 &       593.25 \\
sn2006le   &    54057.275 &       Ks &      2748.74 &       829.45 \\
sn2006le   &    54064.270 &       Ks &      2754.92 &       323.05 \\
sn2006le   &    54078.320 &       Ks &      2788.60 &       623.28 \\
sn2006le   &    54056.279 &       Ks &      2846.49 &       733.11 \\
sn2006le   &    54053.322 &       Ks &      2922.04 &       600.21 \\
sn2006le   &    54045.327 &       Ks &      2924.48 &       674.06 \\
sn2006le   &    54070.206 &       Ks &      2951.29 &       653.68 \\
sn2006le   &    54051.404 &       Ks &      3014.21 &       554.00 \\
sn2006le   &    54044.326 &       Ks &      3098.10 &       504.68 \\
sn2006le   &    54055.395 &       Ks &      3103.45 &       754.76 \\
sn2006le   &    54047.281 &       Ks &      3116.98 &       724.56 \\
sn2006le   &    54077.157 &       Ks &      3135.58 &       607.67 \\
sn2006le   &    54041.353 &       Ks &      3157.26 &       611.46 \\
sn2006le   &    54042.357 &       Ks &      3159.56 &      1206.46 \\
sn2006le   &    54048.290 &       Ks &      3357.65 &       690.15 \\
sn2006le   &    54040.346 &       Ks &      3381.75 &       311.64 \\
sn2006le   &    54043.355 &       Ks &      3677.64 &      1202.61 \\
sn2006le   &    54049.290 &       Ks &      3800.38 &       595.08 \\
sn2006lf   &    54095.161 &        H &       694.12 &       695.73 \\
sn2006lf   &    54100.149 &        H &       785.25 &       795.80 \\
sn2006lf   &    54091.204 &        H &       927.02 &       748.69 \\
sn2006lf   &    54096.126 &        H &       964.02 &       694.43 \\
sn2006lf   &    54094.178 &        H &       980.05 &      1024.64 \\
sn2006lf   &    54154.164 &        H &      -122.27 &       695.74 \\
sn2006lf   &    54153.169 &        H &      -326.00 &       702.44 \\
sn2006lf   &    54093.169 &        H &      1086.92 &       676.58 \\
sn2006lf   &    54083.124 &        H &      1287.36 &       732.42 \\
sn2006lf   &    54090.201 &        H &      1300.17 &       866.89 \\
sn2006lf   &    54085.147 &        H &      1586.73 &       712.71 \\
sn2006lf   &    54082.173 &        H &      1859.12 &       754.67 \\
sn2006lf   &    54086.173 &        H &      1985.00 &       710.78 \\
sn2006lf   &    54081.119 &        H &      2012.96 &       804.26 \\
sn2006lf   &    54080.124 &        H &      2059.37 &       823.81 \\
sn2006lf   &    54079.196 &        H &      2138.17 &       706.29 \\
sn2006lf   &    54084.156 &        H &      2221.98 &       660.01 \\
sn2006lf   &    54076.135 &        H &      2299.16 &       725.60 \\
sn2006lf   &    54078.302 &        H &      2470.65 &       707.37 \\
sn2006lf   &    54077.137 &        H &      2522.61 &      1091.17 \\
sn2006lf   &    54053.458 &        H &      2780.02 &       644.43 \\
sn2006lf   &    54056.258 &        H &      3118.60 &       689.96 \\
sn2006lf   &    54054.307 &        H &      3136.33 &       862.74 \\
sn2006lf   &    54074.166 &        H &      3148.58 &       702.36 \\
sn2006lf   &    54075.171 &        H &      3296.32 &       694.61 \\
sn2006lf   &    54051.383 &        H &      3597.92 &       679.84 \\
sn2006lf   &    54058.190 &        H &      3635.84 &       640.19 \\
sn2006lf   &    54046.287 &        H &      3679.71 &       817.64 \\
sn2006lf   &    54057.191 &        H &      3714.06 &       695.08 \\
sn2006lf   &    54072.173 &        H &      3730.40 &       801.18 \\
sn2006lf   &    54050.285 &        H &      3746.85 &       746.33 \\
sn2006lf   &    54052.257 &        H &      3778.09 &       785.57 \\
sn2006lf   &    54049.268 &        H &      3892.45 &       694.64 \\
sn2006lf   &    54048.269 &        H &      4111.17 &       705.54 \\
sn2006lf   &    54060.230 &        H &      4132.16 &       674.49 \\
sn2006lf   &    54059.288 &        H &      4159.49 &       927.21 \\
sn2006lf   &    54045.307 &        H &      4286.31 &       671.94 \\
sn2006lf   &    54071.210 &        H &      4397.17 &       696.81 \\
sn2006lf   &    54047.260 &        H &      4564.38 &       697.24 \\
sn2006lf   &    54061.224 &        H &      4596.21 &       649.88 \\
sn2006lf   &    54065.181 &        H &      4615.78 &       715.00 \\
sn2006lf   &    54070.186 &        H &      4625.67 &       781.63 \\
sn2006lf   &    54064.204 &        H &      4834.63 &       670.16 \\
sn2006lf   &    54043.334 &        H &      5103.66 &       617.61 \\
sn2006lf   &    54044.305 &        H &      5253.95 &       681.26 \\
sn2006lf   &    54066.179 &        H &      5325.79 &       734.59 \\
sn2006lf   &    54042.336 &        H &      5481.01 &       728.49 \\
sn2006lf   &    54041.332 &        H &      5807.12 &       787.91 \\
sn2006lf   &    54040.325 &        H &      6297.44 &       742.94 \\
sn2006lf   &    54100.149 &        J &        85.43 &       345.54 \\
sn2006lf   &    54154.164 &        J &       -20.15 &       287.84 \\
sn2006lf   &    54153.169 &        J &       -87.99 &       317.63 \\
sn2006lf   &    54095.161 &        J &       203.20 &       297.92 \\
sn2006lf   &    54093.169 &        J &       217.74 &       302.65 \\
sn2006lf   &    54096.126 &        J &       283.28 &       318.23 \\
sn2006lf   &    54082.173 &        J &       297.46 &       230.73 \\
sn2006lf   &    54091.204 &        J &       407.62 &       321.77 \\
sn2006lf   &    54094.178 &        J &       431.21 &       441.71 \\
sn2006lf   &    54084.156 &        J &       485.82 &       296.31 \\
sn2006lf   &    54083.124 &        J &       532.31 &       319.22 \\
sn2006lf   &    54086.173 &        J &       615.98 &       334.54 \\
sn2006lf   &    54090.201 &        J &       619.38 &       379.45 \\
sn2006lf   &    54085.147 &        J &       707.21 &       291.27 \\
sn2006lf   &    54081.119 &        J &       798.00 &       329.68 \\
sn2006lf   &    54079.196 &        J &       967.57 &       312.38 \\
sn2006lf   &    54080.124 &        J &      1027.78 &       354.69 \\
sn2006lf   &    54078.302 &        J &      1068.61 &       327.12 \\
sn2006lf   &    54059.288 &        J &      1089.67 &       389.53 \\
sn2006lf   &    54058.190 &        J &      1133.13 &       302.73 \\
sn2006lf   &    54056.258 &        J &      1205.61 &       313.49 \\
sn2006lf   &    54057.191 &        J &      1216.03 &       313.78 \\
sn2006lf   &    54077.137 &        J &      1234.74 &       475.89 \\
sn2006lf   &    54074.166 &        J &      1259.45 &       293.47 \\
sn2006lf   &    54060.230 &        J &      1266.24 &       324.31 \\
sn2006lf   &    54075.171 &        J &      1302.90 &       301.02 \\
sn2006lf   &    54053.458 &        J &      1340.29 &       312.94 \\
sn2006lf   &    54076.135 &        J &      1352.44 &       338.32 \\
sn2006lf   &    54054.307 &        J &      1459.41 &       383.54 \\
sn2006lf   &    54052.257 &        J &      1664.74 &       292.02 \\
sn2006lf   &    54065.181 &        J &      1673.25 &       338.16 \\
sn2006lf   &    54072.173 &        J &      1822.23 &       328.40 \\
sn2006lf   &    54066.179 &        J &      1936.76 &       340.66 \\
sn2006lf   &    54051.383 &        J &      2027.96 &       351.96 \\
sn2006lf   &    54070.186 &        J &      2238.02 &       366.49 \\
sn2006lf   &    54071.210 &        J &      2292.88 &       329.74 \\
sn2006lf   &    54069.222 &        J &      2475.60 &       555.49 \\
sn2006lf   &    54050.285 &        J &      2737.16 &       338.48 \\
sn2006lf   &    54049.268 &        J &      3242.57 &       360.19 \\
sn2006lf   &    54048.269 &        J &      3519.18 &       354.75 \\
sn2006lf   &    54047.260 &        J &      4241.82 &       350.74 \\
sn2006lf   &    54046.287 &        J &      4646.32 &       337.69 \\
sn2006lf   &    54045.307 &        J &      4871.15 &       343.15 \\
sn2006lf   &    54044.305 &        J &      4995.01 &       350.14 \\
sn2006lf   &    54040.325 &        J &      5419.22 &       404.18 \\
sn2006lf   &    54043.334 &        J &      5468.93 &       305.36 \\
sn2006lf   &    54042.336 &        J &      5651.60 &       408.23 \\
sn2006lf   &    54041.332 &        J &      5828.52 &       424.05 \\
sn2006lf   &    54100.149 &       Ks &       -54.46 &      1178.03 \\
sn2006lf   &    54095.161 &       Ks &       -86.32 &       928.62 \\
sn2006lf   &    54094.178 &       Ks &       348.15 &      1314.90 \\
sn2006lf   &    54090.201 &       Ks &       350.35 &      1217.55 \\
sn2006lf   &    54093.169 &       Ks &       463.95 &      1052.81 \\
sn2006lf   &    54091.204 &       Ks &       676.59 &      1019.45 \\
sn2006lf   &    54086.173 &       Ks &       702.83 &       973.36 \\
sn2006lf   &    54085.147 &       Ks &       798.14 &       992.21 \\
sn2006lf   &    54096.126 &       Ks &       858.52 &      1105.27 \\
sn2006lf   &    54084.156 &       Ks &       879.71 &       941.12 \\
sn2006lf   &    54153.169 &       Ks &      -492.56 &      1063.09 \\
sn2006lf   &    54082.173 &       Ks &      -681.29 &       865.35 \\
sn2006lf   &    54154.164 &       Ks &      -887.17 &       989.05 \\
sn2006lf   &    54083.124 &       Ks &      1138.94 &      1000.57 \\
sn2006lf   &    54077.137 &       Ks &      1408.81 &      1317.72 \\
sn2006lf   &    54076.135 &       Ks &      1481.54 &      1049.89 \\
sn2006lf   &    54080.124 &       Ks &      1523.40 &      1125.95 \\
sn2006lf   &    54081.119 &       Ks &      1842.46 &      1014.08 \\
sn2006lf   &    54079.196 &       Ks &      2251.06 &      1035.90 \\
sn2006lf   &    54075.171 &       Ks &      2524.75 &      1040.65 \\
sn2006lf   &    54078.302 &       Ks &      2615.71 &       965.47 \\
sn2006lf   &    54074.166 &       Ks &      2764.34 &       984.32 \\
sn2006lf   &    54072.173 &       Ks &      3750.42 &      1036.45 \\
sn2006lf   &    54053.458 &       Ks &      3809.21 &      1034.64 \\
sn2006lf   &    54056.258 &       Ks &      3964.90 &       981.19 \\
sn2006lf   &    54071.210 &       Ks &      4006.17 &       959.67 \\
sn2006lf   &    54064.204 &       Ks &      4181.17 &      1005.20 \\
sn2006lf   &    54070.186 &       Ks &      4258.93 &      1064.46 \\
sn2006lf   &    54054.307 &       Ks &      4265.72 &      1257.80 \\
sn2006lf   &    54052.257 &       Ks &      4391.53 &      1034.38 \\
sn2006lf   &    54058.190 &       Ks &      4398.32 &       984.39 \\
sn2006lf   &    54059.288 &       Ks &      4413.80 &      1278.59 \\
sn2006lf   &    54051.383 &       Ks &      4442.60 &      1097.05 \\
sn2006lf   &    54060.230 &       Ks &      4485.83 &      1031.68 \\
sn2006lf   &    54047.260 &       Ks &      4490.02 &      1007.65 \\
sn2006lf   &    54050.285 &       Ks &      4677.21 &      1110.49 \\
sn2006lf   &    54049.268 &       Ks &      4775.67 &      1024.59 \\
sn2006lf   &    54065.181 &       Ks &      5133.20 &      1051.60 \\
sn2006lf   &    54057.191 &       Ks &      5535.46 &       901.78 \\
sn2006lf   &    54048.269 &       Ks &      5610.49 &       996.81 \\
sn2006lf   &    54066.179 &       Ks &      5726.31 &      1063.25 \\
sn2006lf   &    54046.287 &       Ks &      6044.59 &      1046.65 \\
sn2006lf   &    54045.307 &       Ks &      6233.00 &      1031.28 \\
sn2006lf   &    54043.334 &       Ks &      6666.79 &       883.29 \\
sn2006lf   &    54041.332 &       Ks &      6834.61 &      1045.31 \\
sn2006lf   &    54040.325 &       Ks &      6880.86 &      1066.49 \\
sn2006lf   &    54044.305 &       Ks &      7274.75 &       963.68 \\
sn2006lf   &    54042.336 &       Ks &      7998.41 &      1044.40 \\
sn2007co   &    54389.118 &        H &         0.00 &       299.82 \\
sn2007co   &    54278.312 &        H &        45.07 &       177.91 \\
sn2007co   &    54272.291 &        H &        56.11 &       315.67 \\
sn2007co   &    54271.366 &        H &       138.87 &       353.62 \\
sn2007co   &    54282.228 &        H &       192.08 &       250.36 \\
sn2007co   &    54276.250 &        H &       326.81 &       250.14 \\
sn2007co   &    54281.257 &        H &       454.77 &       301.44 \\
sn2007co   &    54285.288 &        H &       475.02 &       178.85 \\
sn2007co   &    54280.190 &        H &      -391.59 &       333.68 \\
sn2007co   &    54273.319 &        H &      -420.55 &       317.56 \\
sn2007co   &    54389.118 &        J &         0.00 &        92.93 \\
sn2007co   &    54276.250 &        J &       301.83 &       103.22 \\
sn2007co   &    54281.257 &        J &       321.05 &       145.97 \\
sn2007co   &    54275.277 &        J &       409.24 &        72.27 \\
sn2007co   &    54278.312 &        J &       439.79 &       136.28 \\
sn2007co   &    54273.319 &        J &       442.31 &       118.06 \\
sn2007co   &    54280.190 &        J &       470.50 &       125.79 \\
sn2007co   &    54285.288 &        J &       504.20 &        95.58 \\
sn2007co   &    54272.291 &        J &       594.79 &        86.97 \\
sn2007co   &    54271.366 &        J &       867.25 &       147.51 \\
sn2007co   &    54389.118 &       Ks &         0.00 &       707.19 \\
sn2007co   &    54276.250 &       Ks &        79.07 &       880.73 \\
sn2007co   &    54280.190 &       Ks &       548.35 &       883.27 \\
sn2007co   &    54272.291 &       Ks &      -462.47 &       589.43 \\
sn2007co   &    54273.319 &       Ks &      -478.75 &       859.64 \\
sn2007co   &    54278.312 &       Ks &      -642.42 &       551.12 \\
sn2007co   &    54285.288 &       Ks &      1654.68 &      1244.86 \\
sn2007co   &    54275.277 &       Ks &     -1110.57 &       502.75 \\
sn2007co   &    54282.228 &       Ks &     -1227.71 &       584.43 \\
sn2007co   &    54271.366 &       Ks &     -1313.35 &       702.04 \\
sn2007co   &    54281.257 &       Ks &     -2336.66 &      1401.22 \\
sn2007cq   &    54384.164 &        H &        46.26 &       120.90 \\
sn2007cq   &    54383.206 &        H &      -542.67 &       414.10 \\
sn2007cq   &    54292.350 &        H &      1042.21 &       242.75 \\
sn2007cq   &    54282.326 &        H &      1098.50 &       375.43 \\
sn2007cq   &    54280.335 &        H &      1199.69 &       351.26 \\
sn2007cq   &    54279.380 &        H &      1289.68 &       262.04 \\
sn2007cq   &    54281.326 &        H &      1710.32 &       325.89 \\
sn2007cq   &    54384.164 &        J &        39.54 &       136.59 \\
sn2007cq   &    54383.206 &        J &       -79.71 &       193.93 \\
sn2007cq   &    54292.350 &        J &       818.13 &       102.72 \\
sn2007cq   &    54282.326 &        J &      2197.03 &       164.92 \\
sn2007cq   &    54281.326 &        J &      2473.11 &       153.73 \\
sn2007cq   &    54280.335 &        J &      2506.56 &        98.68 \\
sn2007cq   &    54279.380 &        J &      2835.96 &       128.39 \\
sn2007cq   &    54384.164 &       Ks &       289.72 &       978.06 \\
sn2007cq   &    54292.350 &       Ks &       924.28 &      1082.86 \\
sn2007cq   &    54383.206 &       Ks &      -404.44 &      1155.60 \\
sn2007cq   &    54280.335 &       Ks &      1445.80 &       777.39 \\
sn2007cq   &    54279.380 &       Ks &      2741.32 &       957.56 \\
sn2007cq   &    54282.328 &       Ks &      2946.40 &      1378.57 \\
\enddata
\tablenotetext{a} {Fluxes are expressed normalized to a zeropoint of 25.  I.e., the calibrated 2MASS magnitude is mag$=-2.5\log_{10}({\rm flux})+25$}
\tablecomments{}
\label{tab:irlcs}
\end{deluxetable}

